Encoding Tight Typing in a Unified Framework

This paper explores how the intersection type theories of call-by-name (CBN) and call-by-value (CBV) can be unified in a more general framework provided by call-by-push-value (CBPV). Indeed, we propose tight type systems for CBN and CBV that can be both encoded in a unique tight type system for CBPV. All such systems are quantitative, ie. they provide exact information about the length of normalization sequences to normal form as well as the size of these normal forms. Moreover, the length of reduction sequences are discriminated according to their multiplicative and exponential nature, a concept inherited from linear logic. Last but not least, it is possible to extract quantitative measures for CBN and CBV from their corresponding encodings in CBPV.

==> proofs/bang/anti-substitution-tight.tex <==
\begin{proof}
By induction on $t$.
\begin{itemize}
  \item $t = x$. Then, $\substitute{x}{u}{t} = u$ and we set $I = \{\ast\}$,
  $\sigma_\ast = \tau$, $\Gamma = \emptyset$ $\Delta_\ast = \Gamma'$, $\Phi^{\ast}_{u} =
  \Phi_{\substitute{x}{u}{t}}$, and
  $\derivable{\Phi_{t}}{\sequT{\assign{x}{\intertype{\tau}{}}}{\assign{x}{\tau}}{0}{0}{0}}{\SysTight}$
  by rule $\ruleBDAxiom$.
  
  \item $t = y \neq x$. Then, $\substitute{x}{u}{t} = y$ and we conclude with
  $I = \emptyset$ (hence, $\intertype{\sigma_i}{i \in I} = \emul$), $\Gamma =
  \Gamma'$ and $\Phi_{t} = \Phi_{\substitute{x}{u}{t}}$. 
  
  \item $t = \termapp{t_1}{t_2}$. Then, $\substitute{x}{u}{t} =
  \termapp{\substitute{x}{u}{t_1}}{\substitute{x}{u}{t_2}}$ and there are three
  possible cases.
  \begin{enumerate}
    \item $\ruleBTArrowE$. Then, $\tau = \typeneutral$, $\Gamma' =
    \ctxtsum{\Gamma'_1}{\Gamma'_2}{}$, $\cmult' = \cmult'_1 + \cmult'_2$,
    $\cexp' = \cexp'_1 + \cexp'_2$ and $\csize' = \csize'_1 + \csize'_2 + 1$
    with premises
    $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t_1}}{\typeneutral}}{\cmult'_1}{\cexp'_1}{\csize'_1}}{\SysTight}$
    and
    $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\Gamma'_2}{\assign{\substitute{x}{u}{t_2}}{\overline{\typeabs}}}{\cmult'_2}{\cexp'_2}{\csize'_2}}{\SysTight}$.
    By \ih on both, there exist type derivations
    $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\typeneutral}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$,
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_1}$,
    $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2;\assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\overline{\typeabs}}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_2}$
    (note that $I_1$ and $I_2$ can be assumed disjoint) such that $\Gamma'_1 =
    \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}$, $\Gamma'_2 =
    \ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}$, $\cmult'_1 = \cmult_1
    +_{i \in I_1}{\cmult_i}$, $\cmult'_2 = \cmult_2 +_{i \in I_2}{\cmult_i}$,
    $\cexp'_1 = \cexp_1 +_{i \in I_1}{\cexp_i}$, $\cexp'_2 = \cexp_2
    +_{i \in I_2}{\cexp_i}$, $\csize'_1 = \csize_1 +_{i \in I_1}{\csize_i}$ and
    $\csize'_2 = \csize_2 +_{i \in I_2}{\csize_i}$. Then, by $\ruleBTArrowE$ we
    have
    $\derivable{\Phi_{t}}{\sequT{\ctxtsum{\Gamma_1}{\Gamma_2}{};\assign{x}{\intertype{\sigma_i}{i \in I_1 \cup I_2}}}{\assign{\termapp{t_1}{t_2}}{\typeneutral}}{\cmult_1+\cmult_2}{\cexp_1+\cexp_2}{\csize_1+\csize_2+1}}{\SysTight}$
    and we conclude with $\Gamma = \ctxtsum{\Gamma_1}{\Gamma_2}{}$, $I = I_1
    \cup I_2$, $\cmult = \cmult_1 + \cmult_2$, $\cexp = \cexp_1 + \cexp_2$ and
    $\csize = \csize_1 + \csize_2 + 1$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtsum{\Gamma'_1}{\Gamma'_2}{} =
       \ctxtsum{\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}}{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{}
       = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult'_1 + \cmult'_2 = \cmult_1
       +_{i \in I_1}{\cmult_i} + \cmult_2 +_{i \in I_2}{\cmult_i} = \cmult
       +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1
       +_{i \in I_1}{\cexp_i} + \cexp_2 +_{i \in I_2}{\cexp_i} = \cexp
       +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize'_1 + \csize'_2 + 1 = \csize_1
       +_{i \in I_1}{\csize_i} + \csize_2 +_{i \in I_2}{\csize_i} + 1 = \csize
       +_{i \in I}{\csize_i}$.
    \end{itemize}
    
    \item $\ruleBDApp$. Then, $\Gamma' =
    \ctxtsum{\Gamma'_1}{\Gamma'_2}{}$, $\cmult' = \cmult'_1 + \cmult'_2 + 1$,
    $\cexp' = \cexp'_1 + \cexp'_2$ and
    $\csize' = \csize'_1 + \csize'_2$
    with premises
    $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t_1}}{\functtype{\M}{\tau}}}{\cmult'_1}{\cexp'_1}{\csize'_1}}{\SysTight}$
    and
    $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\Gamma'_2}{\assign{\substitute{x}{u}{t_2}}{\typeneutral}}{\cmult'_2}{\cexp'_2}{\csize'_2}}{\SysTight}$
    for some multiset type $\M$ such that $\ptight{\M}$. By \ih there
   exist 
    $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\functtype{\M}{\tau}}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$,
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_1}$,
    $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2;\assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\typeneutral}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_2}$
    (note that $I_1$ and $I_2$ can be assumed disjoint)
    such that $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}$, $\Gamma'_2
    = \ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}$, $\cmult'_1 = \cmult_1
    +_{i \in I_1}{\cmult_i}$, $\cmult'_2 = \cmult_2 +_{i \in I_2}{\cmult_i}$,
    $\cexp'_1 = \cexp_1 +_{i \in I_1}{\cexp_i}$, $\cexp'_2 = \cexp_2
    +_{i \in I_2}{\cexp_i}$, $\csize'_1 = \csize_1 +_{i \in I_1}{\csize_i}$ and
    $\csize'_2 = \csize_2 +_{i \in I_2}{\csize_i}$. Then, by $\ruleBDApp$ we
    have the type derivation
    $\derivable{\Phi_{t}}{\sequT{\ctxtsum{\Gamma_1}{\Gamma_2}{};\assign{x}{\intertype{\sigma_i}{i \in I_1 \cup I_2}}}{\assign{\termapp{t_1}{t_2}}{\tau}}{\cmult_1+\cmult_2+1}{\cexp_1+\cexp_2}{\csize_1+\csize_2}}{\SysTight}$
    and we conclude with $\Gamma = \ctxtsum{\Gamma_1}{\Gamma_2}{}$, $I = I_1
    \cup I_2$, $\cmult = \cmult_1 + \cmult_2 + 1$, $\cexp = \cexp_1 + \cexp_2$
    and $\csize = \csize_1 + \csize_2$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtsum{\Gamma'_1}{\Gamma'_2}{} =
       \ctxtsum{\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}}{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{}
       = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult'_1 + \cmult'_2 + 1 = \cmult_1
       +_{i \in I_1}{\cmult_i} + \cmult_2 +_{i \in I_2}{\cmult_i} + 1 = \cmult
       +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1
       +_{i \in I_1}{\cexp_i} + \cexp_2 +_{i \in I_2}{\cexp_i} = \cexp
       +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize'_1 + \csize'_2 = \csize_1
       +_{i \in I_1}{\csize_i} + \csize_2 +_{i \in I_2}{\csize_i} = \csize
       +_{i \in I}{\csize_i}$.
    \end{itemize}
    
    \item $\ruleBDArrowE$. Then, $\Gamma' = \ctxtsum{\Gamma'_1}{\Gamma'_2}{}$,
    $\cmult' = \cmult'_1 + \cmult'_2 + 1$, $\cexp' = \cexp'_1 + \cexp'_2$ and
    $\csize' = \csize'_1 + \csize'_2$ with premises
    $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t_1}}{\functtype{\M}{\tau}}}{\cmult'_1}{\cexp'_1}{\csize'_1}}{\SysTight}$
    and
    $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\Gamma'_2}{\assign{\substitute{x}{u}{t_2}}{\M}}{\cmult'_2}{\cexp'_2}{\csize'_2}}{\SysTight}$
    for some multiset type $\M$. By \ih there exist derivations
    $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\functtype{\M}{\tau}}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$,
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_1}$,
    $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2;\assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\M}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_2}$
    (note that $I_1$ and $I_2$ can be assumed disjoint)
    such that $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}$, $\Gamma'_2
    = \ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}$, $\cmult'_1 = \cmult_1
    +_{i \in I_1}{\cmult_i}$, $\cmult'_2 = \cmult_2 +_{i \in I_2}{\cmult_i}$,
    $\cexp'_1 = \cexp_1 +_{i \in I_1}{\cexp_i}$, $\cexp'_2 = \cexp_2
    +_{i \in I_2}{\cexp_i}$, $\csize'_1 = \csize_1 +_{i \in I_1}{\csize_i}$ and
    $\csize'_2 = \csize_2 +_{i \in I_2}{\csize_i}$. Then, by $\ruleBDArrowE$ we
    obtain the type derivation
    $\derivable{\Phi_{t}}{\sequT{\ctxtsum{\Gamma_1}{\Gamma_2}{};\assign{x}{\intertype{\sigma_i}{i \in I_1 \cup I_2}}}{\assign{\termapp{t_1}{t_2}}{\tau}}{\cmult_1+\cmult_2+1}{\cexp_1+\cexp_2}{\csize_1+\csize_2}}{\SysTight}$
    and we conclude with $\Gamma = \ctxtsum{\Gamma_1}{\Gamma_2}{}$, $I = I_1
    \cup I_2$, $\cmult = \cmult_1 + \cmult_2 + 1$, $\cexp = \cexp_1 + \cexp_2$
    and $\csize = \csize_1 + \csize_2$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtsum{\Gamma'_1}{\Gamma'_2}{} =
       \ctxtsum{\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}}{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{}
       = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult'_1 + \cmult'_2 + 1 = \cmult_1
       +_{i \in I_1}{\cmult_i} + \cmult_2 +_{i \in I_2}{\cmult_i} + 1 = \cmult
       +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1
       +_{i \in I_1}{\cexp_i} + \cexp_2 +_{i \in I_2}{\cexp_i} = \cexp
       +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize'_1 + \csize'_2 = \csize_1
       +_{i \in I_1}{\csize_i} + \csize_2 +_{i \in I_2}{\csize_i} = \csize
       +_{i \in I}{\csize_i}$.
    \end{itemize}
  \end{enumerate}
  
  \item $t = \termabs{y}{t'}$. By $\alpha$-conversion we assume $y \neq x$ and $y
  \notin \fv{u}$. Then, $\substitute{x}{u}{t} =
  \termabs{y}{\substitute{x}{u}{t'}}$ and there are two possible cases.
  \begin{enumerate}
    \item $\ruleBTArrowI$. Then, $\tau = \typeabs$, $\Gamma' =
    \ctxtres{\Gamma'_1}{y}{}$ and $\csize' = \csize'_1 + 1$ with premise
    $\derivable{\Phi_{\substitute{x}{u}{t'}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t'}}{\typetight}}{\cmult'}{\cexp'}{\csize'_1}}{\SysTight}$
    where $\ptight{\Gamma'_1(y)}$ holds. By \ih there exist
    $\derivable{\Phi_{t'}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{t'}{\typetight}}{\cmult}{\cexp}{\csize_1}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I}$
    such that $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I}$, $\cmult' =
    \cmult +_{i \in I}{\cmult_i}$, $\cexp' = \cexp +_{i \in I}{\cexp_i}$ and
    $\csize'_1 = \csize_1 +_{i \in I}{\csize_i}$. Moreover, $y \notin \fv{u}$
    implies $y \notin \dom{\Delta_i}$ for all $i \in I$ and, hence, $\Gamma'_1(y) =
    \Gamma_1(y)$. Then, $\ptight{\Gamma_1(y)}$ holds as well. Finally, by
    $\ruleBTArrowE$ with $y \neq x$ we have
    $\derivable{\Phi_{t}}{\sequT{\ctxtres{\Gamma_1}{y}{};\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{\termabs{y}{t'}}{\typeabs}}{\cmult}{\cexp}{\csize_1+1}}{\SysTight}$
    and we conclude with $\Gamma = \ctxtres{\Gamma_1}{y}{}$ and $\csize =
    \csize_1 + 1$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtres{\Gamma'_1}{y}{} =
       \ctxtres{(\ctxtsum{\Gamma_1}{\Delta_i}{i \in I})}{y}{} =
       \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize'_1 + 1 = \csize_1 +_{i \in I}{\csize_i} + 1 =
       \csize +_{i \in I}{\csize_i}$.
    \end{itemize}
    
    \item $\ruleBDArrowI$. Then, $\tau = \functtype{\Gamma'_1(y)}{\tau'}$,
    $\Gamma' = \ctxtres{\Gamma'_1}{y}{}$ with premise
    $\derivable{\Phi_{\substitute{x}{u}{t'}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t'}}{\tau'}}{\cmult'}{\cexp'}{\csize'}}{\SysTight}$.
    By \ih there exist
    $\derivable{\Phi_{t'}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{t'}{\tau'}}{\cmult}{\cexp}{\csize}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I}$
    such that $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I}$, $\cmult' =
    \cmult +_{i \in I}{\cmult_i}$, $\cexp' = \cexp +_{i \in I}{\cexp_i}$ and
    $\csize' = \csize +_{i \in I}{\csize_i}$. Moreover, $y \notin \fv{u}$
    implies $y \notin \dom{\Delta_i}$ for all $i \in I$ and, hence, $\Gamma'_1(y) =
    \Gamma_1(y)$. Finally, by $\ruleBDArrowE$ with $y \neq x$ we have
    $\derivable{\Phi_{t}}{\sequT{\ctxtres{\Gamma_1}{y}{};\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{\termabs{y}{t'}}{\functtype{\Gamma'_1(y)}{\tau'}}}{\cmult}{\cexp}{\csize}}{\SysTight}$
    and we conclude with $\Gamma = \ctxtres{\Gamma_1}{y}{}$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtres{\Gamma'_1}{y}{} =
       \ctxtres{(\ctxtsum{\Gamma_1}{\Delta_i}{i \in I})}{y}{} =
       \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize +_{i \in I}{\csize_i}$.
    \end{itemize}
  \end{enumerate}
  
  \item $t = \termbang{t'}$. Then, $\substitute{x}{u}{t} =
  \termbang{\substitute{x}{u}{t'}}$ and there are two possible cases.
  \begin{enumerate}
    \item $\ruleBTBang$. Then, $\tau = \typebang$, $\Gamma' = \emptyset$ and 
    $\cmult' = \cexp' = \csize' = 0$. We set $I = \emptyset$ (hence,
    $\intertype{\sigma_i}{i \in I} = \emul$), $\Gamma = \emptyset$ and conclude
    by $\ruleBTBang$ with
    $\derivable{\Phi_{t}}{\sequT{}{\assign{t}{\typebang}}{0}{0}{0}}{\SysTight}$.
    
    \item $\ruleBDBang$. Then, $\tau = \intertype{\tau_j}{j \in J}$,
    $\Gamma' = \ctxtsum{}{\Gamma'_j}{j \in J}$, $\cmult' =
    +_{j \in J}{\cmult'_j}$, $\cexp' = 1 +_{j \in J}{\cexp'_j}$, $\csize' =
    +_{j \in J}{\csize'_j}$ with premise
    $\many{\derivable{\Phi^{j}_{\substitute{x}{u}{t'}}}{\sequT{\Gamma'_j}{\assign{\substitute{x}{u}{t'}}{\tau_j}}{\cmult'_j}{\cexp'_j}{\csize'_j}}{\SysTight}}{j \in J}$.
    By \ih there exist type derivations
    $\derivable{\Phi^{j}_{t'}}{\sequT{\Gamma_j;\assign{x}{\intertype{\sigma_i}{i \in I_j}}}{\assign{t'}{\tau_j}}{\cmult_j}{\cexp_j}{\csize_j}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_j}$
    (note that all $I_j$ can be assumed pairwise disjoint)
    such that $\Gamma'_j = \ctxtsum{\Gamma_j}{\Delta_i}{i \in I_j}$, $\cmult'_j
    = \cmult_j +_{i \in I_j}{\cmult_i}$, $\cexp'_j = \cexp_j
    +_{i \in I_j}{\cexp_i}$ and $\csize'_j = \csize_j +_{i \in I_j}{\csize_i}$
    for each $j \in J$. Then, by $\ruleBDBang$ we have
    $\derivable{\Phi_{t}}{\sequT{\ctxtsum{}{\Gamma_j;\assign{x}{\intertype{\sigma_i}{i \in I_j}}}{j \in J}}{\assign{\termbang{t'}}{\intertype{\tau_j}{j \in J}}}{+_{j \in J}{\cmult_j}}{1+_{j \in J}{\cexp_j}}{+_{j \in J}{\csize_j}}}{\SysTight}$
    and we conclude with $\Gamma = \ctxtsum{}{\Gamma_j}{j \in J}$,
    $I = \bigcup_{j \in J}{I_j}$, $\cmult = +_{j \in J}{\cmult_j}$,
    $\cexp = 1 +_{j \in J}{\cexp_j}$, $\csize = +_{j \in J}{\csize_j}$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtsum{}{\Gamma'_j}{j \in J} =
       \ctxtsum{}{(\ctxtsum{\Gamma_j}{\Delta_i}{i \in I_j})}{j \in J} =
       \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = +_{j \in J}{\cmult'_j} =
       +_{j \in J}{(\cmult_j +_{i \in I_j}{\cmult_i})} = \cmult
       +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = 1 +_{j \in J}{\cexp'_j} = 1
       +_{j \in J}{(\cexp_j +_{i \in I_j}{\cexp_i})} = \cexp
       +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = +_{j \in J}{\csize'_j} =
       +_{j \in J}{(\csize_j +_{i \in I_j}{\csize_i})} = \csize
       +_{i \in I}{\csize_i}$.
    \end{itemize}
  \end{enumerate}
  
  \item $t = \termder{t'}$. Then, $\substitute{x}{u}{t} =
  \termder{(\substitute{x}{u}{t'})}$ and there are two possible cases.
  \begin{enumerate}
    \item $\ruleBTDer$. Then, $\tau = \typeneutral$ and $\csize' = \csize'_1 +
    1$ with
    $\derivable{\Phi_{\substitute{x}{u}{t'}}}{\sequT{\Gamma'}{\assign{\substitute{x}{u}{t'}}{\typeneutral}}{\cmult'}{\cexp'}{\csize'_1}}{\SysTight}$.
    By \ih there exist type derivations
    $\derivable{\Phi_{t'}}{\sequT{\Gamma;\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{t'}{\typeneutral}}{\cmult}{\cexp}{\csize_1}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I}$
    such that $\Gamma' = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$, $\cmult' =
    \cmult +_{i \in I}{\cmult_i}$, $\cexp' = \cexp +_{i \in I}{\cexp_i}$ and
    $\csize'_1 = \csize_1 +_{i \in I}{\csize_i}$. Finally, we conclude by
    $\ruleBTDer$ with
    $\derivable{\Phi_{t}}{\sequT{\Gamma;\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{\termder{t'}}{\typeneutral}}{\cmult}{\cexp}{\csize_1+1}}{\SysTight}$
    and $\csize = \csize_1 + 1$.
    
    \item $\ruleBDDer$. Then, we have the premise
    $\derivable{\Phi_{\substitute{x}{u}{t'}}}{\sequT{\Gamma'}{\assign{\substitute{x}{u}{t'}}{\multiset{\tau}}}{\cmult'}{\cexp'}{\csize'}}{\SysTight}$.
    By \ih there exist type derivations
    $\derivable{\Phi_{t'}}{\sequT{\Gamma;\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{t'}{\multiset{\tau}}}{\cmult}{\cexp}{\csize}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I}$
    such that $\Gamma' = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$, $\cmult' =
    \cmult +_{i \in I}{\cmult_i}$, $\cexp' = \cexp +_{i \in I}{\cexp_i}$ and
    $\csize' = \csize +_{i \in I}{\csize_i}$. Finally, we conclude by
    $\ruleBDDer$ with
    $\derivable{\Phi_{t}}{\sequT{\Gamma;\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{\termder{t'}}{\tau}}{\cmult}{\cexp}{\csize}}{\SysTight}$.
  \end{enumerate}
  
  \item $t = \termsubs{y}{t_2}{t_1}$. By $\alpha$-conversion we assume $y \neq x$,
  $y \notin \fv{t_2}$ and $y \notin \fv{u}$. Then, $\substitute{x}{u}{t} =
  \termsubs{y}{\substitute{x}{u}{t_2}}{\substitute{x}{u}{t_1}}$ and there are two
  possible cases.
  \begin{enumerate}
    \item $\ruleBTESubs$. Then, $\Gamma' =
    \ctxtsum{\ctxtres{\Gamma'_1}{y}{}}{\Gamma'_2}{}$, $\cmult' = \cmult'_1 +
    \cmult'_2$, $\cexp' = \cexp'_1 + \cexp'_2$ and
    $\csize' = \csize'_1 +
    \csize'_2 $ with premises
    $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t_1}}{\tau}}{\cmult'_1}{\cexp'_1}{\csize'_1}}{\SysTight}$
    and
    $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\Gamma'_2}{\assign{\substitute{x}{u}{t_2}}{\typeneutral}}{\cmult'_2}{\cexp'_2}{\csize'_2}}{\SysTight}$
    where $\ptight{\Gamma'_1(y)}$ holds.
    By \ih there exist type derivations
    $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\tau}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$,
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_1}$,
    $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2;\assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\typeneutral}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_2}$
    (note that $I_1$ and $I_2$ can be assumed disjoint)
    such that $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}$, $\Gamma'_2
    = \ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}$, $\cmult'_1 = \cmult_1
    +_{i \in I_1}{\cmult_i}$, $\cmult'_2 = \cmult_2 +_{i \in I_2}{\cmult_i}$,
    $\cexp'_1 = \cexp_1 +_{i \in I_1}{\cexp_i}$, $\cexp'_2 = \cexp_2
    +_{i \in I_2}{\cexp_i}$, $\csize'_1 = \csize_1 +_{i \in I_1}{\csize_i}$ and
    $\csize'_2 = \csize_2 +_{i \in I_2}{\csize_i}$. Moreover, $y \notin \fv{u}$
    implies $y \notin \dom{\Delta_i}$ for all $i \in I_1 \cup I_2$ while $y \notin
    \fv{t_2}$ implies $y \notin \dom{\Gamma_2}$. Hence, $\Gamma'_1(y) = \Gamma_1(y)$
    and $\ptight{\Gamma_1(y)}$ holds as well. Finally, by $\ruleBTESubs$ with
    $y \neq x$ we have
    $\derivable{\Phi_{t}}{\sequT{\ctxtsum{\ctxtres{\Gamma_1}{y}{}}{\Gamma_2}{};\assign{x}{\intertype{\sigma_i}{i \in I_1 \cup I_2}}}{\assign{\termsubs{y}{t_2}{t_1}}{\tau}}{\cmult_1+\cmult_2}{\cexp_1+\cexp_2}{\csize_1+\csize_2}}{\SysTight}$
    and we conclude with $\Gamma =
    \ctxtsum{\ctxtres{\Gamma_1}{y}{}}{\Gamma_2}{}$, $I = I_1 \cup I_2$, $\cmult =
    \cmult_1 + \cmult_2$, $\cexp = \cexp_1 + \cexp_2$ and $\csize = \csize_1 +
    \csize_2 $ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtsum{\ctxtres{\Gamma'_1}{y}{}}{\Gamma'_2}{} =
       \ctxtsum{\ctxtres{(\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1})}{y}{}}{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{}
       $, and this last context is equal to $\ctxtsum{\ctxtsum{\ctxtres{\Gamma_1}{y}{}}{\Gamma_2}{}}{\Delta_i}{i \in I}
       = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult'_1 + \cmult'_2 = \cmult_1
       +_{i \in I_1}{\cmult_i} + \cmult_2 +_{i \in I_2}{\cmult_i} = \cmult
       +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1
       +_{i \in I_1}{\cexp_i} + \cexp_2 +_{i \in I_2}{\cexp_i} = \cexp
       +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize'_1 + \csize'_2 = \csize_1
       +_{i \in I_1}{\csize_i} + \csize_2 +_{i \in I_2}{\csize_i} = \csize
       +_{i \in I}{\csize_i}$.
    \end{itemize}
    
    \item $\ruleBDESubs$. Then, $\Gamma' =
    \ctxtsum{\ctxtres{\Gamma'_1}{y}{}}{\Gamma'_2}{}$, $\cmult' = \cmult'_1 +
    \cmult'_2$, $\cexp' = \cexp'_1 + \cexp'_2$ and $\csize' = \csize'_1 +
    \csize'_2$ with premises
    $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\Gamma'_1}{\assign{\substitute{x}{u}{t_1}}{\tau}}{\cmult'_1}{\cexp'_1}{\csize'_1}}{\SysTight}$
    and
    $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\Gamma'_2}{\assign{\substitute{x}{u}{t_2}}{\Gamma'_1(y)}}{\cmult'_2}{\cexp'_2}{\csize'_2}}{\SysTight}$.
    Thus, by \ih there exist type derivations
    $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\tau}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$,
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_1}$,
    $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2;\assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\Gamma'_1(y)}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
    and
    $\many{\derivable{\Phi^{i}_{u}}{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTight}}{i \in I_2}$
    (note that $I_1$ and $I_2$ can be assumed disjoint)
    such that $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}$, $\Gamma'_2
    = \ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}$, $\cmult'_1 = \cmult_1
    +_{i \in I_1}{\cmult_i}$, $\cmult'_2 = \cmult_2 +_{i \in I_2}{\cmult_i}$,
    $\cexp'_1 = \cexp_1 +_{i \in I_1}{\cexp_i}$, $\cexp'_2 = \cexp_2
    +_{i \in I_2}{\cexp_i}$, $\csize'_1 = \csize_1 +_{i \in I_1}{\csize_i}$ and
    $\csize'_2 = \csize_2 +_{i \in I_2}{\csize_i}$. Moreover, $y \notin \fv{u}$
    implies $y \notin \dom{\Delta_i}$ for all $i \in I_1 \cup I_2$ while $y \notin
    \fv{t_2}$ implies $y \notin \dom{\Gamma_2}$. Hence, $\Gamma'_1(y) = \Gamma_1(y)$.
    Finally, by $\ruleBDESubs$ with $y \neq x$ we have
    $\derivable{\Phi_{t}}{\sequT{\ctxtsum{\ctxtres{\Gamma_1}{y}{}}{\Gamma_2}{};\assign{x}{\intertype{\sigma_i}{i \in I_1 \cup I_2}}}{\assign{\termsubs{y}{t_2}{t_1}}{\tau}}{\cmult_1+\cmult_2}{\cexp_1+\cexp_2}{\csize_1+\csize_2}}{\SysTight}$
    and we conclude with $\Gamma =
    \ctxtsum{\ctxtres{\Gamma_1}{y}{}}{\Gamma_2}{}$, $I = I_1 \cup I_2$, $\cmult =
    \cmult_1 + \cmult_2$, $\cexp = \cexp_1 + \cexp_2$ and $\csize = \csize_1 +
    \csize_2$ since:
    \begin{itemize}
       \item $\Gamma' = \ctxtsum{\ctxtres{\Gamma'_1}{y}{}}{\Gamma'_2}{} =
       \ctxtsum{\ctxtres{(\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1})}{y}{}}{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{}
       $ and this last context is equal to $
       \ctxtsum{\ctxtsum{\ctxtres{\Gamma_1}{y}{}}{\Gamma_2}{}}{\Delta_i}{i \in I}
       = \ctxtsum{\Gamma}{\Delta_i}{i \in I}$.
       
       \item $\cmult' = \cmult'_1 + \cmult'_2 = \cmult_1
       +_{i \in I_1}{\cmult_i} + \cmult_2 +_{i \in I_2}{\cmult_i} = \cmult
       +_{i \in I}{\cmult_i}$.
       
       \item $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1
       +_{i \in I_1}{\cexp_i} + \cexp_2 +_{i \in I_2}{\cexp_i} = \cexp
       +_{i \in I}{\cexp_i}$.
       
       \item $\csize' = \csize'_1 + \csize'_2 = \csize_1
       +_{i \in I_1}{\csize_i} + \csize_2 +_{i \in I_2}{\csize_i} = \csize
       +_{i \in I}{\csize_i}$.
    \end{itemize}
  \end{enumerate}
\end{itemize}
\end{proof}


==> proofs/bang/anti-substitution.tex <==
\begin{proof}
By induction on $t$.
\comment{
\begin{itemize}
  \item $t = x$. Then, $\substitute{x}{u}{t} = u$ and we set 
  $I = \{1\}$, $\sigma_1 = \tau$, $\Gamma = \emptyset$ $\Delta_1 = \Gamma'$,
  $\Phi^{1}_{u} = \Phi_{\substitute{x}{u}{t}}$, and
  $\derivable{\Phi_t}{\sequB{\assign{x}{\intertype{\tau}{}}}{\assign{x}{\tau}}}{\SysBang}$
  by rule $\ruleBAxiom$. We conclude since $\size{\Phi_t} = |I| = 1$.
  
  \item $t = y \neq x$. Then, $\substitute{x}{u}{t} = y$ and
  we conclude with $I = \emptyset$ (hence, $\intertype{\sigma_i}{i \in I} =
  \emul$), $\Gamma = \Gamma'$ and $\Phi_t =
  \Phi_{\substitute{x}{u}{t}}$. 
  
  
  \item $t = \termapp{s}{r}$. Then, $\substitute{x}{u}{t} =
  \termapp{\substitute{x}{u}{s}}{\substitute{x}{u}{r}}$. Moreover, by rule
  $\ruleBArrowE$, $\Gamma' = \ctxtsum{\Gamma'_1}{\Gamma'_2}{}$ s.t.
  $\derivable{\Phi_{\substitute{x}{u}{s}}}{\sequB{\Gamma'_1}{\assign{\substitute{x}{u}{s}}{\functtype{\M}{\tau}}}}{\SysBang}$
  and
  $\derivable{\Phi_{\substitute{x}{u}{r}}}{\sequB{\Gamma'_2}{\assign{\substitute{x}{u}{r}}{\M}}}{\SysBang}$.
  By \ih on $\Phi_{\substitute{x}{u}{s}}$ there exist derivations
  $\derivable{\Phi_s}{\sequB{\Gamma_1; \assign{x}{\intertype{\sigma_i}{i \in
  I_s}}}{\assign{s}{\functtype{\M}{\tau}}}}{\SysBang}$ and
  $\many{\derivable{\Phi^i_u}{\sequB{\Delta_i}{\assign{u}{\sigma_i}}}{\SysBang}}{i
  \in I_s}$ s.t. $\Gamma'_1 = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_s}$ and
  $\size{\Phi_{\substitute{x}{u}{s}}} = \size{\Phi_{s}}  +_{i \in
  I_s}{\size{\Phi^i_{u}}} - |I_s|$. By \ih once again, this time on
  $\Phi_{\substitute{x}{u}{r}}$, there exists $\derivable{\Phi_r}{\sequB{\Gamma_2;
  \assign{x}{\intertype{\sigma_i}{i \in I_r}}}{\assign{s}{\M}}}{\SysBang}$ and
  $\many{\derivable{\Phi^i_u}{\sequB{\Delta_i}{\assign{u}{\sigma_i}}}{\SysBang}}{i
  \in I_r}$ such that $\Gamma'_r = \ctxtsum{\Gamma_1}{\Delta_i}{i \in I_r}$ and
  $\size{\Phi_{\substitute{x}{u}{r}}} = \size{\Phi_{r}}  +_{i \in
  I_r}{\size{\Phi^i_{u}}} - |I_r|$. Consider $I = I_s \cup I_r$. Then, by rule
  $\ruleBArrowE$, \[
  \Rule{\derivable{\Phi_s}{\sequB{\Gamma_1; \assign{x}{\intertype{\sigma_i}{i \in I_s}}}{\assign{s}{\functtype{\M}{\tau}}}}{\SysBang}
        \quad
        \derivable{\Phi_r}{\sequB{\Gamma_2; \assign{x}{\intertype{\sigma_i}{i \in I_r}}}{\assign{s}{\M}}}{\SysBang}}
       {\sequB{\ctxtsum{\Gamma_1}{\Gamma_2}{}; \assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{\termapp{s}{r}}{\tau}}}
       {\ruleBArrowE} \]
  Moreover, we have \[
  \begin{array}{rcl}
  \size{\Phi_{\substitute{x}{u}{t}}}
    & = & \size{\Phi_{\substitute{x}{u}{s}}} + \size{\Phi_{\substitute{x}{u}{r}}} + 1 \\
    & = & \size{\Phi_{s}}  +_{i \in I_s}{\size{\Phi^i_{u}}} - |I_s| + \size{\Phi_{r}}  +_{i \in I_r}{\size{\Phi^i_{u}}} - |I_r| + 1 \\
    & = & \size{\Phi_{s}} + \size{\Phi_{r}} + 1  +_{i \in I}{\size{\Phi^i_{u}}} - |I| \\
    & = & \size{\Phi_{t}} +_{i \in I}{\size{\Phi^i_{u}}} - |I| 
  \end{array} \] and
  $\many{\derivable{\Phi^i_u}{\sequB{\Delta_i}{\assign{u}{\sigma_i}}}{\SysBang}}{i
  \in I}$. Thus, we conclude.
  
  \item The remaining inductive cases are similar, concluding directly from
  the \ih
\end{itemize}
}
\end{proof}



==> proofs/bang/clash-free-czero-tight.tex <==
\begin{proof}
We proceed by induction on the derivation of  $\cfnrml{t}$ (resp. $\cfntrl{t}$,
$\cfnbang{t}$ and $\cfnabs{t}$). Moreover, we generalise the statement and
simultaneously show the following:
\begin{enumerate}
  \item\label{l:typing-normal-clash-free:ne} If $\cfntrl{t}$, then $\sigma = \typeneutral$; 
  \item\label{l:typing-normal-clash-free:nb} If $\cfnbang{t}$, then $\sigma \in \overline{\typebang}$;
  \item\label{l:typing-normal-clash-free:na} If $\cfnabs{t}$, then $\sigma \in \overline{\typeabs}$.
\end{enumerate}

We analyse the possible cases for $t$.
\begin{itemize}
  \item Let $\cfntrl{x}$, so that $\wsize{x} = 0$. Then, take
  $\derivable{}{\sequT{\assign{x}{\multiset{\typeneutral}}}{\assign{x}{\typeneutral}}{0}{0}{0}}{\SysTight}$
  to conclude.

  \item Let $\cfntrl{\termder{t}}$ with $\cfntrl{t}$. Then, apply the
  \ih (\ref{l:typing-normal-clash-free:ne}) to obtain
  $\derivable{}{\sequT{\Gamma}{\assign{t}{\typeneutral}}{0}{0}{\wsize{t}}}{\SysTight}$
  and conclude 
  $\derivable{}{\sequT{\Gamma}{\assign{\termder{t}}{\typeneutral}}{0}{0}{\wsize{t} + 1}}{\SysTight}$
  with rule $\ruleBTDer$. The size is as expected since $\wsize{\termder{t}} =
  \wsize{t} + 1$.
  
  \item Let $\cfntrl{\termapp{t}{u}}$ with $\cfntrl{t}$ and $\cfnabs{u}$.
  Then, apply the \ih (\ref{l:typing-normal-clash-free:ne}) and
  (\ref{l:typing-normal-clash-free:na}) to obtain
  $\derivable{}{\sequT{\Gamma}{\assign{t}{\typeneutral}}{0}{0}{\wsize t}}{\SysTight}$
  and
  $\derivable{}{\sequT{\Delta}{\assign{u}{\overline \typeabs}}{0}{0}{\wsize{u}}}{\SysTight}$
  resp., and conclude
  $\derivable{}{\sequT{\ctxtsum{\Gamma}{\Delta}{}}{\assign{\termapp{t}{u}}{\typeneutral}}{0}{0}{\wsize{t} + \wsize{u} + 1}}{\SysTight}$
  with rule $\ruleBTArrowE$. The size is as expected since
  $\wsize{\termapp{t}{u}} = \wsize{t} + \wsize{u} + 1$.
  
  \item Let $\cfntrl{\termsubs{x}{u}{t}}$ with $\cfntrl{t}$ and $\cfntrl{u}$,
  or $\cfnabs{\termsubs{x}{u}{t}}$ with $\cfnabs{t}$ and $\cfntrl{u}$, or
  $\cfnbang{\termsubs{x}{u}{t}}$ with $\cfnbang{t}$ and $\cfntrl{u}$.
  Then, apply the appropriate \ih to obtain
  $\derivable{}{\sequT{\Gamma}{\assign{t}{\typetight}}{0}{0}{\wsize{t}}}{\SysTight}$
  and
  $\derivable{}{\sequT{\Delta}{\assign{u}{\typeneutral}}{0}{0}{\wsize{u}}}{\SysTight}$,
  and conclude
  $\derivable{}{\sequT{\ctxtsum{(\ctxtres{\Gamma}{x}{})}{\Delta}{}}{\assign{\termsubs{x}{u}{t}}{\typetight}}{0}{0}{\wsize{t} + \wsize{u}}}{\SysTight}$
  by rule $\ruleBTESubs$ since $\Gamma(x)$ is tight. The size is as expected
  since $\wsize{\termsubs{x}{u}{t}} = \wsize{t} + \wsize{u}$.
  
  \item Let $\cfnabs{\termbang{t}}$. Then, conclude
  $\derivable{}{\sequT{}{\assign{\termbang{t}}{\typebang}}{0}{0}{0}}{\SysTight}$
  by $\ruleBTBang$. The size is as expected.
  
  \item Let $\cfnbang{\termabs{x}{t}}$ with $\cfnrml{t}$. Then, apply the
  appropriate \ih to obtain
  $\derivable{}{\sequT{\Gamma}{\assign{t}{\typetight}}{0}{0}{\wsize{t}}}{\SysTight}$
  and conclude
  $\derivable{}{\sequT{\ctxtres{\Gamma}{x}{}}{\assign{\termabs{x}{t}}{\typeabs}}{0}{0}{\wsize{t} + 1}}{\SysTight}$
  by $\ruleBTArrowI$ since $\Gamma(x)$ is tight.
\end{itemize}
\end{proof}



==> proofs/bang/clash-free-tight.tex <==
\begin{proof}
Similar to Thm.~\ref{t:clashfree-bang} using Lem.~\ref{l:clashfree-tight}. Note
that the consuming rules of system $\SysTight$ are essentially the typing
rules of system $\SysBang$. 
\end{proof}



==> proofs/bang/clash-free.tex <==
\begin{proof}
By simultaneous induction on the following claims: 
\begin{enumerate}
  \item\label{t:clashfree-bang:ne} $\cfntrl{t}$ iff $\pntrl{t}$ and for every
  type $\tau$ we have
  $\derivable{}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysBang}$.
  
  \item\label{t:clashfree-bang:na} $\cfnabs{t}$ iff $\pnabs{t}$ and
  $\derivable{}{\sequB{\Gamma}{\assign{t}{\M}}}{\SysBang}$.
  
  \item\label{t:clashfree-bang:nb} $\cfnbang{t}$ iff $\pnbang{t}$ and
  $\derivable{}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysBang}$.
  
  \item\label{t:clashfree-bang:no} $\cfnrml{t}$ iff $\pnrml{t}$ and
  $\derivable{}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysBang}$.
\end{enumerate}
We first show the left-to-right implications by only analysing the key cases.
If $t = \cfntrl{x}$, then $\pntrl{t}$ and for every type $\tau$ we conclude by
$\ruleBAxiom$. If $t = \cfntrl{\termapp{s}{u}}$, by definition $\cfntrl{s}$
and $\cfnabs{u}$. Let $\tau$ be any type. By \ih (\ref{t:clashfree-bang:na})
$\pnabs{u}$ and $\derivable{}{\sequB{\Delta}{\assign{u}{\M}}}{\SysBang}$. Then,
by \ih (\ref{t:clashfree-bang:ne}) we get $\pntrl{s}$ and
$\derivable{}{\sequB{\Gamma}{\assign{s}{\functtype{\M}{\tau}}}}{\SysBang}$.
Moreover, $\pntrl{s}$ and $\pnabs{u}$ imply $\pnabs{s}$ and $\pnrml{u}$ resp.,
hence $\pntrl{t}$. Thus, we conclude by $\ruleBArrowE$,
$\derivable{}{\sequB{\ctxtsum{\Gamma}{\Delta}{}}{\assign{\termapp{s}{u}}{\tau}}}{\SysBang}$.
If $t = \cfnbang{\termabs{x}{s}}$, then $\cfnrml{s}$ by definition. By \ih
(\ref{t:clashfree-bang:no}) $\pnrml{s}$ and
$\derivable{}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}$ for some type
$\tau$. Then, $\pnbang{t}$ and we conclude by $\ruleBArrowI$,
$\derivable{}{\sequB{\ctxtres{\Gamma}{x}{}}{\assign{\termabs{x}{s}}{\functtype{\Gamma(x)}{\tau}}}}{\SysBang}$.
If $t = \cfnabs{\termbang{s}}$, then $\pnabs{t}$ by definition and we conclude
by $\ruleBBang$,
$\derivable{}{\sequB{}{\assign{\termbang{s}}{\emul}}}{\SysBang}$. If $t =
\cfntrl{\termder{s}}$, then $\cfntrl{s}$ by definition. Let $\tau$ be any
type, by \ih (\ref{t:clashfree-bang:ne}) we get $\pntrl{s}$ and
$\derivable{}{\sequB{\Gamma}{\assign{s}{\multiset{\tau}}}}{\SysBang}$.
Moreover, $\pntrl{s}$ implies $\pnbang{s}$ and hence $\pntrl{t}$. Thus, we
conclude by $\ruleBDer$,
$\derivable{}{\sequB{\Gamma}{\assign{\termder{s}}{\tau}}}{\SysBang}$. If $t =
\termsubs{x}{u}{s}$, then $\cfntrl{u}$ and there are three possible cases:
$\cfntrl{s}$, $\cfnabs{s}$ or $\cfnbang{s}$. In either case, by the proper \ih
we get $\derivable{}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}$ (resp. $\M$)
and conclude by $\ruleBESubs$, given that \ih (\ref{t:clashfree-bang:ne}) on
$u$ implies $\pntrl{u}$ and
$\derivable{}{\sequB{\Delta}{\assign{u}{\Gamma(x)}}}{\SysBang}$. Note that
$\pntrl{u}$ in turn implies $\pnbang{u}$, thus $t$ remains in the same set as
$s$ ($\ipntrl$, $\ipnabs$ or $\ipnbang$ resp.).

The right-to-left implications uses Lem.~\ref{l:clashfree-bang}.  
\end{proof}


==> proofs/bang/completeness-tight.tex <==
\begin{proof}
We prove the statement for $\loredn$ and then conclude for the general notion
of reduction $\rewrite{\bangweak}$ by Thm.~\ref{t:confluence}. Let
$t \loredn^{(\cmult,\cexp)} p$. We proceed by induction on $\cmult+\cexp$.

If $\cmult+\cexp = 0$, then $\cmult = \cexp = 0$ and thus $t = p$, which
implies $\cfnrml{t}$. Lem.~\ref{l:typing-normal-clash-free} allows to
conclude.

If $\cmult+\cexp > 0$, then there exists $t'$ such that $t \lored^{(1,0)} t'
\loredn^{(\cmult-1,\cexp)} p$ or $t \lored^{(0,1)} t'
\loredn^{(\cmult,\cexp-1)} p$. By \ih there exists a tight derivation
$\derivable{\Phi'}{\sequT{\Gamma}{\assign{t'}{\sigma}}{\cmult'}{\cexp'}{\wsize{p}}}{\SysTight}$
such that $\cmult' + \cexp' = \cmult + \cexp -1$. Lem.~\ref{l:QSE-tight} gives a
tight derivation
$\derivable{\Phi}{\sequT{\Gamma}{\assign{t}{\sigma}}{\cmult''}{\cexp''}{\wsize{p}}}{\SysTight}$
such that $\cmult'' + \cexp'' = \cmult' + \cexp' + 1$. We then have $\cmult'' +
\cexp'' = \cmult + \cexp$. The fact that $\cmult'' = \cmult$ and $\cexp'' =
\cexp$ holds by a simple case analysis.
\end{proof}



==> proofs/bang/correctness-tight.tex <==
\begin{proof}
We prove the statement by showing that $t \loredn^{(\cmult,\cexp)} p$ holds for
the deterministic strategy, then we conclude since $\lored \mathbin{\subseteq}
\rewrite{\bangweak}$. Let
$\derivable{\Phi}{\sequT{\Gamma}{\assign{t}{\sigma}}{\cmult}{\cexp}{\csize}}{\SysTight}$.
We reason by induction on $\cmult+\cexp$.

If $\cmult+\cexp = 0$, then $\cmult = \cexp = 0$ and Lem.~\ref{l:czero-normal}
gives $\pnrml{t}$. Moreover, by Lem.~\ref{l:tight-size} and
Thm.~\ref{t:clashfree-tight}, we get both $\wsize{t} = \csize$ and
$\cfnrml{t}$. Thus, we conclude with $p = t$.

If $\cmult+\cexp > 0$, then $t \notin \ipnrml$ holds by
Lem.~\ref{l:czero-normal} and thus there exists $t'$ such that $t \lored^{(1,0)} t'$
or $t \lored^{(0,1)} t'$
by Prop.~\ref{l:cbn-cbv-normal-forms}. By Lem.~\ref{l:QSR} there is
$\derivable{\Phi'}{\sequT{\Gamma}{\assign{t'}{\sigma}}{\cmult'}{\cexp'}{\csize}}{\SysTight}$
such that $1 + \cmult' + \cexp' = \cmult + \cexp$. By the \ih there is $p$ such
that $\cfnrml{p}$ and $t' \loredn^{(\cmult',\cexp')} p$
with $\csize = \wsize{p}$. Then $t \lored^{(1,0)} t' \loredn^{(\cmult',\cexp')} p$
(resp. $t \lored^{(0,1)} t' \ldots$)
which means $t \loredn^{(\cmult,\cexp)} p$, as expected.
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> proofs/bang/czero-normal.tex <==
\begin{proof}
$\left.\Rightarrow\right)$ By induction on $\Phi$.
\begin{itemize}
  \item $\ruleBDAxiom$. Then $t = x$, $\Gamma = \intertype{\sigma}{}$ with
  $\sigma \in \typetight$. By definition $\pntrl{t}$ holds, which implies
  $\pnrml{t}$ as well.
  
  \item $\ruleBTArrowE$. Then $t = \termapp{r}{u}$, $\sigma = \typeneutral$,
  $\Gamma = \ctxtsum{\Gamma'}{\Delta}{}$, $\csize = \csize' + \csize'' + 1$,
  $\sequT{\Gamma'}{\assign{r}{\typeneutral}}{0}{0}{\csize'}$,
  $\sequT{\Delta}{\assign{u}{\overline{\typeabs}}}{0}{0}{\csize''}$. Then,
  $\Gamma'$ and $\Delta$ are both tight, hence the \ih gives $\pnrml{r}$ and 
  $\pnrml{u}$. There are two cases to consider based on $\pnrml{r}$:
  \begin{enumerate}
    \item if $\pnabs{r}$ the result is immediate.

    \item if $\pnbang{r}$ then we can assume $r \notin \ipnabs$ too (since
    $\pnabs{r}$ is already considered). Then, by Rem.~\ref{r:normal},
    $\pabs{r}$ holds. This leads to a contradiction with $r$ having type
    $\typeneutral$ (\cf Rem.~\ref{r:typing}). Hence, this case does not apply.
  \end{enumerate}
  
  \item $\ruleBDApp$. This case does not apply since it concludes
  with $\cmult > 0$.
  
  \item $\ruleBDArrowE$. This case does not apply since it concludes
  with $\cmult > 0$.
  
  \item $\ruleBTArrowI$. Then $t = \termabs{x}{u}$, $\sigma = \typeabs$, $\Gamma
  = \ctxtres{\Gamma'}{x}{}$, $\csize = \csize' + 1$,
  $\sequT{\Gamma'}{\assign{u}{\typetight}}{0}{0}{\csize'}$ and
  $\ptight{\Gamma'(x)}$. Since $\Gamma$ is tight and $\ptight{\Gamma'(x)}$,
  $\Gamma'$ is tight as well. Then, by \ih $\pnrml{u}$ holds, which implies
  $\pnrml{t}$ too.
  
  \item $\ruleBDArrowI$. Then $\sigma = \functtype{\M}{\tau}$ which
  contradicts the hypothesis of $\Phi$ being tight. Hence, this case does not
  apply.
  
  \item $\ruleBTBang$. Then $t = \termbang{u}$ which implies $\pnabs{t}$ and
  hence $\pnrml{t}$.
  
  \item $\ruleBDBang$. This case does not apply since it concludes with
  $\cexp > 0$.
  
  \item $\ruleBTDer$. Then $t = \termder{u}$, $\sigma = \typeneutral$,
  $\csize = \csize' + 1$ and
  $\sequT{\Gamma}{\assign{u}{\typeneutral}}{0}{0}{\csize'}$. By \ih $\pnrml{u}$
  holds. There are two  cases to consider:
  \begin{enumerate}
    \item if $\pnbang{u}$ the result is immediate.
    
    \item if $\pnabs{u}$ and $u \notin \ipnbang$, then $\pbang{u}$ holds by
    Rem.~\ref{r:normal}. This leads to a contradiction with $u$ having type
    $\typeneutral$ (\cf Rem.~\ref{r:typing}). Hence, this case does not apply.
  \end{enumerate}
  
  \item $\ruleBDDer$. Then $t = \termder{u}$ and
  $\derivable{\Phi_u}{\sequT{\Gamma}{\assign{u}{\intertype{\sigma}{}}}{0}{0}{\csize}}{\SysTight}$.
  Then, Lem.~\ref{l:tight-spreading-czero} on $\Phi_u$ give
  $\intertype{\sigma}{} \in \typetight$ which is clearly a contradiction. Thus,
  this case does not apply.
  
  \item $\ruleBTESubs$. Then $t = \termsubs{x}{u}{r}$, $\Gamma =
    \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$,
    $\csize = \csize' + \csize''$, $\sequT{\Gamma'}{\assign{r}{\sigma}}{0}{0}{\csize'}$,
  $\sequT{\Delta}{\assign{u}{\typeneutral}}{0}{0}{\csize''}$ and
  $\ptight{\Gamma'(x)}$. Since $\Gamma$ is tight and $\ptight{\Gamma'(x)}$,
  then $\Gamma'$ and $\Delta$ are both tight as well. Thus, \ih gives
  $\pnrml{r}$ and $\pnrml{u}$. Moreover, by definition $\pnrml{r}$ means
  $\pnabs{r}$ or $\pnbang{r}$. Same for $\pnrml{u}$, hence there are two
  different cases to analyse:
  \begin{enumerate}
    \item if $\pnbang{u}$ the result is immediate.
    \item if $\pnabs{u}$ and $u \notin \ipnbang$, then $\pbang{u}$ holds by
    Rem.~\ref{r:normal}. This leads to a contradiction with $u$ having type
    $\typeneutral$ (\cf Rem.~\ref{r:typing}). Hence, this case does not apply.
  \end{enumerate}
  
  \item $\ruleBDESubs$. Then $t = \termsubs{x}{u}{r}$, $\csize = \csize' +
  \csize''$ and $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$ tight
  such that, in particular,
  $\derivable{\Phi_u}{\sequT{\Delta}{\assign{u}{\Gamma'(x)}}{0}{0}{\csize''}}{\SysTight}$
  with $\Delta$ tight. By Lem.~\ref{l:tight-spreading-czero} on $\Phi_u$,
  $\Gamma'(x) \in \typetight$ which leads to a contradiction, since
  $\Gamma'(x)$ is a multiset type by definition. Hence, this case does not apply.
\end{itemize}

$\left.\Leftarrow\right)$ By induction on $t$.
\begin{itemize}
  \item $t = x$. Then, $\Phi$ ends with rule $\ruleBDAxiom$ and the statement holds
  trivially.
  
  \item $t = \termapp{r}{u}$. By definition $\pnrml{t}$ gives $\pnabs{r}$ and
  $\pnrml{u}$. Thus, $\pnrml{r}$ holds too. There are three  cases to consider:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTArrowE$, then $\sigma =
    \typeneutral$, $\Gamma = \ctxtsum{\Gamma'}{\Delta}{}$, $\cmult = \cmult' +
    \cmult''$, $\cexp = \cexp' + \cexp''$, $\csize = \csize' + \csize'' + 1$,
    $\sequT{\Gamma'}{\assign{r}{\typeneutral}}{\cmult'}{\cexp'}{\csize'}$,
    $\sequT{\Delta}{\assign{u}{\overline{\typeabs}}}{\cmult''}{\cexp''}{\csize''}$.
    Moreover, $\Gamma'$ and $\Delta$ are both tight. Then, the \ih with
    $\pnrml{r}$ and $\pnrml{u}$ gives $\cmult' = \cexp' = 0$ and $\cmult'' =
    \cexp'' = 0$. Hence, $\cmult = \cexp = 0$.
    
    \item if $\Phi$ ends with rule $\ruleBDArrowE$, then $\Gamma =
    \ctxtsum{\Gamma'}{\Delta}{}$, $\cmult = \cmult' + \cmult'' + 1$,
    $\cexp = \cexp' + \cexp''$, $\csize = \csize' + \csize''$ and, in
    particular,
    $\derivable{\Phi_r}{\sequT{\Gamma'}{\assign{r}{\functtype{\M}{\tau}}}{\cmult'}{\cexp'}{\csize'}}{\SysTight}$.
    Moreover, by contra-positive of Rem.~\ref{r:typing} with $\Phi_r$, it is
    necessarily the case $\neg \pbang{r}$. Thus, together with $\pnabs{r}$ it
    gives $\pntrl{r}$ (\cf Rem.~\ref{r:normal}). Also,
    $\Gamma$ tight implies $\Gamma'$ tight as well. Then, by
    Lem.~\ref{l:tight-spreading-neutral}, $\Phi_r$ is a tight typing, which
    leads to a contradiction with $r$ having a functional type. Hence, this
    case does not apply.

    \item if $\Phi$ ends with rule $\ruleBDApp$, then $\Gamma =
    \ctxtsum{\Gamma'}{\Delta}{}$, $\cmult = \cmult' + \cmult'' +1$, $\cexp =
    \cexp' + \cexp''$,
    $\csize = \csize' + \csize''$ and, in particular,
    $\derivable{\Phi_r}{\sequT{\Gamma'}{\assign{r}{\functtype{\M}{\typetight}}}{\cmult'}{\cexp'}{\csize'}}{\SysTight}$.
    This case is identical to the previous one.
    \end{enumerate}
  
  \item $t = \termabs{x}{u}$. By definition $\pnrml{t}$ gives $\pnrml{u}$.
  There are two cases to consider for $\Phi$:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTArrowI$, then $\sigma = \typeabs$,
    $\Gamma = \ctxtres{\Gamma'}{x}{}$, $\csize = \csize' + 1$,
    $\derivable{\Phi_u}{\sequT{\Gamma'}{\assign{u}{\typetight}}{\cmult}{\cexp}{\csize'}}{\SysTight}$
    and $\ptight{\Gamma'(x)}$. Since $\Gamma$ is tight and
    $\ptight{\Gamma'(x)}$, $\Gamma'$ is tight as well. Then, the \ih gives
    $\cmult = \cexp = 0$.
    
    \item if $\Phi$ ends with rule $\ruleBDArrowI$, then $\sigma =
    \functtype{\M}{\tau}$ which contradicts the hypothesis of $\Phi$ being
    tight. Hence, this case does not apply.
  \end{enumerate}
  
  \item $t = \termbang{u}$. There are two cases to consider for $\Phi$:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTBang$, then $\cmult = \cexp = 0$ and
    the statement holds immediately.
    
    \item if $\Phi$ ends with rule $\ruleBDBang$, then $\sigma$ is a multiset
    type which contradicts the hypothesis of $\Phi$ being tight. Hence, this
    case does not apply.
  \end{enumerate}
  
  \item $t = \termder{u}$. By definition $\pnrml{t}$ gives $\pnbang{u}$ which
  implies $\pnrml{u}$ as well. There are two cases to consider:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTDer$, then $\sigma = \typeneutral$,
    $\csize = \csize' + 1$ and
    $\sequT{\Gamma}{\assign{u}{\typeneutral}}{\cmult}{\cexp}{\csize'}$. Then,
    the statement follows immediately from the \ih
    
    \item if $\Phi$ ends with rule $\ruleBDDer$, then
    $\derivable{\Phi_u}{\sequT{\Gamma}{\assign{u}{\intertype{\sigma}{}}}{\cmult}{\cexp}{\csize}}{\SysTight}$.
    Moreover, by contra-positive of Rem.~\ref{r:typing} with $\Phi_u$, it is
    necessarily the case $\neg\pabs{u}$. Thus, together with $\pnbang{u}$ it
    gives $\pntrl{u}$ (\cf Rem.~\ref{r:normal}). Then, by
    Lem.~\ref{l:tight-spreading-neutral}, $\Phi_u$ is a tight typing, which
    leads to a contradiction with $u$ having a multiset type. Hence, this case
    does not apply.
  \end{enumerate}
  
  \item $t = \termsubs{x}{u}{r}$. By definition $\pnrml{t}$ implies $\pnrml{r}$
  and $\pnbang{u}$, which in turn implies $\pnrml{u}$ as well. Then, there are
  two cases to consider for $\Phi$:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTESubs$, then $\sigma \in \typetight$,
    $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$, $\cmult = \cmult'
      + \cmult''$, $\cexp = \cexp' + \cexp''$,
      $\csize = \csize' + \csize''$,
    $\sequT{\Gamma'}{\assign{r}{\sigma}}{\cmult'}{\cexp'}{\csize'}$,
    $\sequT{\Delta}{\assign{u}{\typeneutral}}{\cmult''}{\cexp''}{\csize''}$ and
    $\ptight{\Gamma'(x)}$. Since $\Gamma$ is tight and $\ptight{\Gamma'(x)}$,
    then $\Gamma'$ and $\Delta$ are both tight as well. Then, the \ih with
    $\pnrml{r}$ and $\pnrml{u}$ gives $\cmult' = \cexp' = 0$ and $\cmult'' =
    \cexp'' = 0$. Hence, $\cmult = \cexp = 0$.
    
    \item if $\Phi$ ends with rule $\ruleBDESubs$, then $\cmult = \cmult' +
    \cmult''$, $\cexp = \cexp' + \cexp''$, $\csize = \csize' + \csize''$ and
    $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$ tight such that, in
    particular,
    $\derivable{\Phi_u}{\sequT{\Delta}{\assign{u}{\Gamma'(x)}}{\cmult''}{\cexp''}{\csize''}}{\SysTight}$
    with $\Delta$ tight. Moreover, by contra-positive of Rem.~\ref{r:typing}
    with $\Phi_u$, it is necessarily the case $\neg\pabs{u}$. Thus, together
    with $\pnbang{u}$ it gives $\pntrl{u}$ (\cf Rem.~\ref{r:normal}). Then, by
    Lem.~\ref{l:tight-spreading-neutral}, $\Phi_u$ is a tight typing, which
    leads to a contradiction with $u$ having a multiset type. Hence, this case
    does not apply.
  \end{enumerate}
\end{itemize}
\end{proof}


==> proofs/bang/subject-expansion-tight.tex <==
\begin{proof}
By induction on $t \lored t'$.
\begin{itemize}
  \item $t = \termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{u} \lored
  \ctxtapp{\ctxt{L}}{\termsubs{x}{u}{s}} = t'$. We reason by induction on
  $\ctxt{L}$.
  \begin{itemize}
    \item $\ctxt{L} = \Box$. There are two cases depending on the last rule
    of $\Phi'$.
    \begin{enumerate}
      \item $\ruleBTESubs$. Then, $\Phi'$ has the following form: \[
\Rule{
  \sequT{\Gamma'}{\assign{s}{\typetight}}{\cmult_s}{\cexp_s}{\csize_s}
  \quad
  \sequT{\Delta}{\assign{u}{\typeneutral}}{\cmult_u}{\cexp_u}{\csize_u}
  \quad
  \ptight{\Gamma'(x)}
}{
  \sequT{\ctxtsum{\ctxtres{\Gamma'}{x}{}}{\Delta}{}}{\assign{\termsubs{x}{u}{s}}{\typetight}}{\cmult_s+\cmult_u}{\cexp_s+\cexp_u}{\csize_s+\csize_u}
}{\ruleBTESubs}
      \] We can then construct the following derivation $\Phi$: \[\kern-4em
\Rule{
  \Rule{
    \sequT{\Gamma'}{\assign{s}{\typetight}}{\cmult_s}{\cexp_s}{\csize_s}
  }{
    \sequT{\ctxtres{\Gamma'}{x}{}}{\assign{\termabs{x}{s}}{\functtype{\Gamma'(x)}{\typetight}}}{\cmult_s}{\cexp_s}{\csize_s}
  }{\ruleBDArrowI}
  \quad
  \sequT{\Delta}{\assign{u}{\typeneutral}}{\cmult_u}{\cexp_u}{\csize_u}
  \quad
  \ptight{\Gamma'(x)}
}{
  \sequT{\ctxtsum{\ctxtres{\Gamma'}{x}{}}{\Delta}{}}{\assign{\termapp{(\termabs{x}{s})}{u}}{\typetight}}{\cmult_s+\cmult_u+1}{\cexp_s+\cexp_u}{\csize_s+\csize_u}
}{\ruleBDApp}
      \] The counters verify the expected property.
      
      \item $\ruleBDESubs$. Then, $\Phi'$ has the following form: \[
\Rule{
  \sequT{\Gamma'}{\assign{s}{\tau}}{\cmult_s}{\cexp_s}{\csize_s}
  \quad
  \sequT{\Delta}{\assign{u}{\Gamma'(x)}}{\cmult_u}{\cexp_u}{\csize_u}
}{
  \sequT{\ctxtsum{\ctxtres{\Gamma'}{x}{}}{\Delta}{}}{\assign{\termsubs{x}{u}{s}}{\tau}}{\cmult_s+\cmult_u}{\cexp_s+\cexp_u}{\csize_s+\csize_u}
}{\ruleBDESubs}
      \] We can then construct the following derivation $\Phi$: \[
\Rule{
  \Rule{
    \sequT{\Gamma'}{\assign{s}{\tau}}{\cmult_s}{\cexp_s}{\csize_s}
  }{
    \sequT{\ctxtres{\Gamma'}{x}{}}{\assign{\termabs{x}{s}}{\functtype{\Gamma'(x)}{\tau}}}{\cmult_s}{\cexp_s}{\csize_s}
  }{\ruleBDArrowI}
  \quad
  \sequT{\Delta}{\assign{u}{\Gamma'(x)}}{\cmult_u}{\cexp_u}{\csize_u}
}{
  \sequT{\ctxtsum{\ctxtres{\Gamma'}{x}{}}{\Delta}{}}{\assign{\termapp{(\termabs{x}{s})}{u}}{\tau}}{\cmult_s+\cmult_u+1}{\cexp_s+\cexp_u}{\csize_s+\csize_u}
}{\ruleBDArrowE}
      \] The counters verify the expected property.
    \end{enumerate}
    
    \item $\ctxt{L}= \termsubs{y}{r}{\ctxt{L'}}$. Immediate from the \ih
  \end{itemize}
  
  \item $t = \termsubs{x}{\ctxtapp{\ctxt{L}}{\termbang{u}}}{s} \lored
  \ctxtapp{\ctxt{L}}{\substitute{x}{u}{s}} = t'$. We reason by induction on
  $\ctxt{L}$.
  \begin{itemize}
    \item $\ctxt{L} = \Box$. Then $\Phi$ has the form
    $\sequT{\Gamma}{\assign{\substitute{x}{u}{s}}{\sigma}}{\cmult'}{\cexp'}{\csize}$.
    By Lem.~\ref{l:bang:anti-substitution-tight} there exist
    $\sequT{\Gamma';\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{s}{\sigma}}{\cmult_s}{\cexp_s}{\csize_s}$
    and
    $\many{\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i}}{i \in I}$
    such that $\Gamma = \ctxtsum{\Gamma'}{\Delta_i}{i \in I}$,
    $\cmult' = \cmult_s +_{i \in I}{\cmult_i}$, $\cexp' = \cexp_s +_{i \in I}{\cexp_i}$ and
    $\csize = \csize_s +_{i \in I}{\csize_i}$.
    We can then construct the following derivation $\Phi$: \[\kern-2em
\Rule{
  \sequT{\Gamma';\assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{s}{\sigma}}{\cmult_s}{\cexp_s}{\csize_s}
  \quad
  \Rule{
    (\sequT{\Delta_i}{\assign{u}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i})_{i \in I}
  }{
    \sequT{\ctxtsum{}{\Delta_i}{i \in I}}{\assign{\termbang{u}}{\intertype{\sigma_i}{i \in I}}}{+_{i \in I}{\cmult_i}}{1+_{i \in I}{\cexp_i}}{+_{i \in I}{\csize_i}}
  }{\ruleBDBang}
}{
  \sequT{\ctxtsum{\Gamma'}{\Delta_i}{i \in I}}{\assign{\termsubs{x}{\termbang{u}}{s}}{\sigma}}{\cmult_s+_{i \in I}{\cmult_i}}{1+\cexp_s+_{i \in I}{\cexp_i}}{\csize_s+_{i \in I}{\csize_i}}
}{\ruleBDESubs}
    \] The counters verify the expected property.
    
    \item $\ctxt{L}= \termsubs{y}{r}{\ctxt{L'}}$. Immediate from the \ih
  \end{itemize}
  
  \item $t=\termder{(\ctxtapp{\ctxt{L}}{\termbang{s}})} \lored \ctxtapp{\ctxt{L}}{s} = t'$. We reason by induction on $\ctxt{L}$.
  \begin{itemize}
    \item $\ctxt{L} = \Box$. Then, $t' = s$ and from $\Phi'$ we construct the
    following derivation: \[
\Rule{
  \Rule{
    \sequT{\Gamma}{\assign{s}{\sigma}}{\cmult'}{\cexp'}{\csize}
  }{
    \sequT{\Gamma}{\assign{\termbang{s}}{\intertype{\sigma}{}}}{\cmult'}{1+\cexp'}{\csize}
  }{\ruleBDBang}
}{
  \sequT{\Gamma}{\assign{\termder{\termbang{s}}}{\sigma}}{\cmult'}{1+\cexp'}{\csize}}{\ruleBDDer}
    \] We conclude since the counters verify the expected property.
    
    \item $\ctxt{L}= \termsubs{y}{u}{\ctxt{L'}}$. Immediate from the \ih
  \end{itemize}
  
  \item All the inductive cases for internal reductions are straightforward by \ih
  \end{itemize}
\end{proof}


==> proofs/bang/subject-expansion.tex <==
\begin{proof}

By induction on the context $\ctxt{S}$ where the rewriting rule ($\dBeta$,
$\sBang$ or $\dBang$) is being applied in $t \rewrite{\bangweak} t'$.
\begin{itemize}
  \item $\ctxt{S} = \Box$. Then, we have one case per rewriting rule:
  \begin{itemize}
    \item Rule $\dBeta$. Then, $t =
    \termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{u}$ and $t' =
    \ctxtapp{\ctxt{L}}{\termsubs{x}{u}{s}}$. We proceed by induction on
    $\ctxt{L}$.
    \begin{itemize}
      \item $\ctxt{L} = \Box$. Then, $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$ such
      that \[
      \Rule{\derivable{\Phi'_s}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}
            \quad
            \derivable{\Phi'_u}{\sequB{\Delta}{\assign{u}{\Gamma'(x)}}}{\SysBang}
           }
           {\derivable{\Phi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}}{\assign{\termsubs{x}{u}{s}}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] then, we construct \[
      \Rule{\Rule{\derivable{\Phi'_s}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}}
                 {\sequB{\ctxtres{\Gamma'}{x}{}}{\assign{\termabs{x}{s}}{\functtype{\Gamma'(x)}{\tau}}}}
                 {\ruleBArrowI}
            \quad
            \derivable{\Phi'_u}{\sequB{\Delta}{\assign{u}{\Gamma'(x)}}}{\SysBang}
           }
           {\derivable{\Phi}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}}{\assign{\termapp{(\termabs{x}{s})}{u}}{\tau}}}{\SysBang}}
           {\ruleBArrowE} \]
      Note that $\size{\Phi} = \size{\Phi'} + 1$.
      
      \item $\ctxt{L} = \termsubs{y}{r}{\ctxt{L'}}$. Then, $\Gamma =
      \ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}$ such that \[
      \Rule{\derivable{\Psi'}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termsubs{x}{u}{s}}}{\tau}}}{\SysBang}
            \quad
            \derivable{\Phi'_r}{\sequB{\Delta}{\assign{r}{\Gamma'(y)}}}{\SysBang}
           }
           {\derivable{\Phi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}}{\assign{\termsubs{y}{r}{\ctxtapp{\ctxt{L'}}{\termsubs{x}{u}{s}}}}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] By \ih on $\Psi'$ we have a derivation
      $\derivable{\Psi}{\sequB{\Gamma'}{\assign{\termapp{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{u}}{\tau}}}{\SysBang}$
      with $\size{\Psi} > \size{\Psi'}$.
      Moreover, by rule $\ruleBArrowE$, $\Gamma' =
      \ctxtsum{\Gamma'_1}{\Gamma'_2}{}$ and \[
      \Rule{\derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'_1}{\assign{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{\functtype{\M}\tau}}}{\SysBang}
            \quad
            \derivable{\Phi_u}{\sequB{\Gamma'_2}{\assign{u}{\M}}}{\SysBang}
           }
           {\derivable{\Psi}{\sequB{\Gamma'}{\assign{\termapp{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{u}}{\tau}}}{\SysBang}}
           {\ruleBArrowE}
      \] Moreover, by hypothesis of rule $\dB$, $y \notin \fv{u}$. Thus, in
      particular, $y \notin \dom{\Gamma'_2}$ and $\Gamma'(y) = \Gamma'_1(y)$.
      Then, we construct %{\scriptsize
      \[\kern-5em
      \Rule{\Rule{\derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'_1}{\assign{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{\functtype{\M}\tau}}}{\SysBang}
                  \quad
                  \derivable{\Phi'_r}{\sequB{\Delta}{\assign{r}{\Gamma'_1(y)}}}{\SysBang}
                 }
                 {\sequB{\ctxtsum{(\ctxtres{\Gamma'_1}{y}{})}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{\functtype{\M}{\tau}}}}
                 {\ruleBESubs}
            \quad
            \derivable{\Phi_u}{\sequB{\Gamma'_2}{\assign{u}{\M}}}{\SysBang}
           }
           {\derivable{\Phi}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}}{\assign{\termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{u}}{\tau}}}{\SysBang}}
           {\ruleBArrowE}
      \] %}
      and conclude with \[
      \begin{array}{rcl}
      \size{\Phi} & = & \size{\Phi_{\ctxt{L'}}} + \size{\Phi'_r} + 1 + \size{\Phi_u} + 1 \\
                  & = & \size{\Psi} + \size{\Phi'_r} + 1 \\
                  & > & \size{\Psi'} + \size{\Phi'_r} + 1 \\
                  & = & \size{\Phi'}
      \end{array} \]
    \end{itemize}
    
    \item Rule $\sBang$. Then, $t =
    \termsubs{x}{\ctxtapp{\ctxt{L}}{\termbang{u}}}{s}$ and $t' =
    \ctxtapp{\ctxt{L}}{\substitute{x}{u}{s}}$. We proceed by induction on
    $\ctxt{L}$.
    \begin{itemize}
      \item $\ctxt{L} = \Box$. By Lem.~\ref{l:antisubstitution-bang} with
      $\Phi'$, there exist 
      $\derivable{\Phi_s}{\sequB{\Gamma'; \assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{s}{\tau}}}{\SysBang}$
      and
      $\many{\derivable{\Phi^i_u}{\sequB{\Delta_i}{\assign{u}{\sigma_i}}}{\SysBang}}{i \in I}$
      such that $\Gamma = \ctxtsum{\Gamma'}{\Delta_i}{i \in I}$ and
      $\size{\Phi'} = \size{\Phi_{s}} + \sum_{i \in
      I}{\size{\Phi^i_{u}}} - |I|$. Then, we construct \[
      \Rule{\derivable{\Phi_s}{\sequB{\Gamma'; \assign{x}{\intertype{\sigma_i}{i \in I}}}{\assign{s}{\tau}}}{\SysBang}
            \quad
            \Rule{\many{\derivable{\Phi^i_u}{\sequB{\Delta_i}{\assign{u}{\sigma_i}}}{\SysBang}}{i \in I}}
                 {\sequB{\ctxtsum{}{\Delta_i}{i \in I}}{\assign{\termbang{u}}{\intertype{\sigma_i}{i \in I}}}}
                 {\ruleBBang}
           }
           {\derivable{\Phi}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] and conclude since $\size{\Phi} = \size{\Phi_s} + \sum_{i \in
      I}{\size{\Phi^i_{u}}} + 2 > \size{\Phi'}$.
      
      \item $\ctxt{L} = \termsubs{y}{r}{\ctxt{L'}}$. Then, $\Gamma =
      \ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}$ such that \[
      \Rule{\derivable{\Psi'}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\substitute{x}{u}{s}}}{\tau}}}{\SysBang}
            \quad
            \derivable{\Phi'_r}{\sequB{\Delta}{\assign{r}{\Gamma'(y)}}}{\SysBang}
           }
           {\derivable{\Phi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}}{\assign{\termsubs{y}{r}{\ctxtapp{\ctxt{L'}}{\substitute{x}{u}{s}}}}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] By \ih on $\Psi'$ we have a derivation
      $\derivable{\Psi}{\sequB{\Gamma'}{\assign{\termsubs{x}{\ctxtapp{\ctxt{L'}}{\termbang{u}}}{s}}{\tau}}}{\SysBang}$
      with $\size{\Psi} > \size{\Psi'}$. Moreover, by rule $\ruleBESubs$,
      $\Gamma' = \ctxtsum{\Gamma'_1}{\Gamma'_2}{}$ and \[
      \Rule{\derivable{\Phi_s}{\sequB{\Gamma'_1}{\assign{s}{\tau}}}{\SysBang}
            \quad
            \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'_2}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{u}}}{\Gamma'_1(x)}}}{\SysBang}
           }
           {\derivable{\Psi}{\sequB{\Gamma'}{\assign{\termsubs{x}{\ctxtapp{\ctxt{L'}}{\termbang{u}}}{s}}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] Moreover, by hypothesis of rule $\sBang$, $y \notin \fv{s}$. Thus, in
      particular, $y \notin \dom{\Gamma'_1}$ and $\Gamma'(y) = \Gamma'_2(y)$.
      Then, we construct \[\kern-1em
      \Rule{\derivable{\Phi_s}{\sequB{\Gamma'_1}{\assign{s}{\tau}}}{\SysBang}
            \quad
            \Rule{\derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'_2}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{u}}}{\Gamma'_1(x)}}}{\SysBang}
                  \quad
                  \derivable{\Phi'_r}{\sequB{\Delta}{\assign{r}{\Gamma'_2(y)}}}{\SysBang}
                 }
                 {\sequB{\ctxtsum{(\ctxtres{\Gamma'_2}{y}{})}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L}}{\termbang{u}}}{\Gamma'_1(x)}}}
                 {\ruleBESubs}
           }
           {\derivable{\Phi}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] and conclude with \[
      \begin{array}{rcl}
      \size{\Phi} & = & \size{\Phi_s} + \size{\Phi_{\ctxt{L'}}} + \size{\Phi'_r} + 2 \\
                  & = & \size{\Psi} + \size{\Phi'_r} + 1 \\
                  & > & \size{\Psi'} + \size{\Phi'_r} + 1 \\
                  & = & \size{\Phi'}
      \end{array} \]
    \end{itemize}
    
    \item Rule $\dBang$. Then, $t =
    \termder{(\ctxtapp{\ctxt{L}}{\termbang{s}})}$ and $t' =
    \ctxtapp{\ctxt{L}}{s}$. We proceed by induction on $\ctxt{L}$.
    \begin{itemize}
      \item $\ctxt{L} = \Box$. We have a derivation
      $\derivable{\Phi'}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}$ and we
      construct \[
      \Rule{\Rule{\derivable{\Phi'}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}}
                 {\sequB{\Gamma}{\assign{\termbang{s}}{\intertype{\tau}{}}}}
                 {\ruleBBang}
           }
           {\derivable{\Phi}{\sequB{\Gamma}{\assign{\termder{(\termbang{s})}}{\tau}}}{\SysBang}}
           {\ruleBDer}
      \] to conclude since $\size{\Phi} = \size{\Phi'} + 2$.
      
      \item $\ctxt{L} = \termsubs{y}{r}{\ctxt{L'}}$. Then, $\Gamma =
      \ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}$ such that \[
      \Rule{\derivable{\Psi'}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{s}}{\tau}}}{\SysBang}
            \quad
            \derivable{\Phi'_r}{\sequB{\Delta}{\assign{r}{\Gamma'(y)}}}{\SysBang}
           }
           {\derivable{\Phi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}}{\assign{\termsubs{y}{r}{\ctxtapp{\ctxt{L'}}{s}}}{\tau}}}{\SysBang}}
           {\ruleBESubs}
      \] By \ih on $\Psi'$ we have a derivation
      $\derivable{\Psi}{\sequB{\Gamma'}{\assign{\termder{(\ctxtapp{\ctxt{L'}}{\termbang{s}})}}{\tau}}}{\SysBang}$
      with $\size{\Psi} > \size{\Psi'}$. Moreover, by rule $\ruleBDer$, \[
      \Rule{\derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{s}}}{\intertype{\tau}{}}}}{\SysBang}}
           {\derivable{\Psi}{\sequB{\Gamma'}{\assign{\termder{(\ctxtapp{\ctxt{L'}}{\termbang{s}})}}{\tau}}}{\SysBang}}
           {\ruleBDer}
      \] Then, we construct \[
      \Rule{\Rule{\derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{s}}}{\intertype{\tau}{}}}}{\SysBang}
                  \quad
                  \derivable{\Phi'_r}{\sequB{\Delta}{\assign{r}{\Gamma'(y)}}}{\SysBang}
                 }
                 {\sequB{\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L}}{\termbang{s}}}{\intertype{\tau}{}}}}
                 {\ruleBESubs}
           }
           {\derivable{\Phi}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysBang}}
           {\ruleBDer}
      \] and conclude with \[
      \begin{array}{rcl}
      \size{\Phi} & = & \size{\Phi_{\ctxt{L'}}} + \size{\Phi'_r} + 2 \\
                  & = & \size{\Psi} + \size{\Phi'_r} + 1 \\
                  & > & \size{\Psi'} + \size{\Phi'_r} + 1 \\
                  & = & \size{\Phi'}
      \end{array} \]
    \end{itemize}
  \end{itemize}
  
  \item All the inductive cases for $\ctxt{S}$ are straightforward by the \ih
\end{itemize}
\end{proof}



==> proofs/bang/subject-reduction-tight.tex <==
\begin{proof}
By induction on $t \lored t'$.
\begin{itemize}
  \item $t = \termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{u}}}{r} \lored
  \ctxtapp{\ctxt{L}}{\termsubs{x}{r}{u}} = t'$. We reason by induction on
  $\ctxt{L}$.
  \begin{itemize}
    \item $\ctxt{L} = \Box$. We first remark that $\Phi$ cannot end with rule
    $\ruleBTArrowE$ since $\termabs{x}{u}$ cannot be typed with $\typeneutral$,
    then there are two cases depending on the last rule of $\Phi$.
    \begin{enumerate}
      \item If $\Phi$ has the following form: \[
\Rule{
  \Rule{
    \sequT{\Gamma_u;\assign{x}{\M}}{\assign{u}{\tau}}{\cmult_u}{\cexp_u}{\csize_u}
  }{
    \sequT{\Gamma_u}{\assign{\termabs{x}{u}}{\functtype{\M}{\tau}}}{\cmult_u}{\cexp_u}{\csize_u}
  }{\ruleBDArrowI}
  \quad
  \sequT{\Gamma_r}{\assign{r}{\M}}{\cmult_r}{\cexp_r}{\csize_r}
}{
  \sequT{\ctxtsum{\Gamma_u}{\Gamma_r}{}}{\assign{\termapp{(\termabs{x}{u})}{r}}{\tau}}{\cmult_u+\cmult_r+1}{\cexp_u+\cexp_r}{\csize_u+\csize_r}
}{\ruleBDArrowE}
      \] We can then construct the following derivation $\Phi'$. \[
\Rule{
  \sequT{\Gamma_u;\assign{x}{\M}}{\assign{u}{\tau}}{\cmult_u}{\cexp_u}{\csize_u}
  \quad
  \sequT{\Gamma_r}{\assign{r}{\M}}{\cmult_r}{\cexp_r}{\csize_r}
}{
  \sequT{\ctxtsum{\Gamma_u}{\Gamma_r}{}}{\assign{\termsubs{x}{r}{u}}{\tau}}{\cmult_u+\cmult_r}{\cexp_u+\cexp_r}{\csize_u+\csize_r}
}{\ruleBDESubs}
      \] The counters verify the expected property. 

      \item If $\Phi$ has the following form: \[\kern-2em
\Rule{
  \Rule{
    \sequT{\Gamma_u;\assign{x}{\M}}{\assign{u}{\typetight}}{\cmult_u}{\cexp_u}{\csize_u}
  }{
    \sequT{\Gamma_u}{\assign{\termabs{x}{u}}{\functtype{\M}{\typetight}}}{\cmult_u}{\cexp_u}{\csize_u}
  }{\ruleBDArrowI}
  \quad
  \sequT{\Gamma_{r}}{\assign{r}{\typeneutral}}{\cmult_r}{\cexp_r}{\csize_r}
  \quad
  \ptight{\M}
}{
  \sequT{\ctxtsum{\Gamma_u}{\Gamma_r}{}}{\assign{\termapp{(\termabs{x}{u})}{r}}{\typetight}}{\cmult_u+\cmult_r+1}{\cexp_u+\cexp_r}{\csize_u+\csize_r}
}{\ruleBDApp}
      \] We can then construct the following derivation $\Phi'$. \[
\Rule{
  \sequT{\Gamma_u;\assign{x}{\M}}{\assign{u}{\typetight}}{\cmult_u}{\cexp_u}{\csize_u}
  \quad
  \sequT{\Gamma_r}{\assign{r}{\typeneutral}}{\cmult_r}{\cexp_r}{\csize_r}
  \quad
  \ptight{\M}
}{
  \sequT{\ctxtsum{\Gamma_u}{\Gamma_{r}}{}}{\assign{\termsubs{x}{r}{u}}{\typetight}}{\cmult_u+\cmult_r}{\cexp_u+\cexp_r}{\csize_u+\csize_r}
}{\ruleBTESubs}
      \] The counters verify the expected property.
    \end{enumerate}
    
    \item $\ctxt{L} = \termsubs{x}{t}{\ctxt{L'}}$. Immediate from the \ih
  \end{itemize}
  
  \item $t = \termsubs{x}{\ctxtapp{\ctxt{L}}{\termbang{r}}}{u}
  \lored \ctxtapp{\ctxt{L}}{\substitute{x}{r}{u}} = t'$. We reason by induction
  on $\ctxt{L}$.
  \begin{itemize}
    \item $\ctxt{L} = \Box$. We first remark that $\Phi$ cannot end with
    rule $\ruleBTESubs$ since $\termbang{r}$ cannot be typed with
    $\typeneutral$, then $\Phi$ has the following form: \[\kern-3em
\Rule{
  \sequT{\Gamma_u; x: \intertype{\sigma_i}{\iI}}{\assign{u}{\sigma}}{\cmult_u}{\cexp_u}{\csize_u}
  \quad
  \Rule{(\sequT{\Gamma_i}{\assign{r}{\sigma_i}}{\cmult_i}{\cexp_i}{\csize_i})_{\iI}}{\sequT{\ctxtsum{}{\Gamma_i}{i \in I}}{\assign{\termbang{r}}{\intertype{\sigma_i}{\iI}}}{+_{\iI} \cmult_i}{1 +_{\iI} \cexp_i}{+_{\iI}\csize_i}}{\ruleBDBang}
}{
  \sequT{\ctxtsum{\Gamma_u}{\Gamma_i}{i \in I}}{\assign{\termsubs{x}{\termbang{r}}{u}}{\sigma}}{\cmult_u +_{\iI} \cmult_i}{\cexp_u +1 +_{\iI} \cexp_i }{\csize_u +_{\iI} \csize_i}
}{\ruleBDESubs}
    \] By applying Lem.~\ref{l:substitution-tight} to the premises we obtain a
    derivation \[
\derivable{\Phi'}{\sequT{\ctxtsum{\Gamma_u}{\Gamma_i}{i \in I}}{\assign{\substitute{x}{r}{u}}{\sigma}}{\cmult_u+_{\iI}{\cmult_i}}{\cexp_u+_{\iI}{\cexp_i}}{\csize_u+_{\iI}{\csize_i}}}{}
    \] The counters verify the expected property.
    
    \item $\ctxt{L}= \termsubs{x}{t}{\ctxt{L'}}$. Immediate from the \ih
  \end{itemize}

  \item $t = \termder{(\ctxtapp{\ctxt{L}}{\termbang{u}})} \lored
  \ctxtapp{\ctxt{L}}{u}=t'$. We reason by induction on $\ctxt{L}$.
  \begin{itemize}
    \item $\ctxt{L} = \Box$. Then $\Phi$ has necessarily the following form: \[
\Rule{
  \Rule{
    \sequT{\Gamma_u}{\assign{u}{\sigma}}{\cmult_u}{\cexp_u}{\csize_u}
  }{
    \sequT{\Gamma_u}{\assign{\termbang{u}}{\intertype{\sigma}{}}}{\cmult_u}{1+\cexp_u}{\csize_u}
  }{\ruleBDBang}
}{
  \sequT{\Gamma_u}{\assign{\termder{\termbang{u}}}{\sigma}}{\cmult_u}{1+\cexp_u}{\csize_u}
}{\ruleBDDer}
    \] We conclude with the derivation $\Phi'$ given by the premise. The
    counters verify the expected property.
    
    \item $\ctxt{L} = \termsubs{x}{t}{\ctxt{L'}}$. Immediate from the \ih
  \end{itemize}
  
  \item All the inductive cases for internal reductions are straightforward by \ih
\end{itemize}  
\end{proof}


==> proofs/bang/subject-reduction.tex <==
\begin{proof}
By induction on the context $\ctxt{S}$ where the rewriting rule ($\dBeta$,
$\sBang$ or $\dBang$) is being applied. 
\begin{itemize}
  \item $\ctxt{S} = \Box$. Then we have one case per rewriting rule:
  \begin{itemize}
    \item Rule $\dBeta$. Then $t = \termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{u}$
    and $t' = \ctxtapp{\ctxt{L}}{\termsubs{x}{u}{s}}$. We proceed by induction
    on $\ctxt{L}$.
    \begin{itemize}
      \item $\ctxt{L} = \Box$. Then $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$
      s.t. $\Gamma'(x) = \M$ and $$
\Rule{
  \Rule{
    \derivable{\Phi_{s}}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}
  }{
    \sequB{\ctxtres{\Gamma'}{x}{}}{\assign{\termabs{x}{s}}{\functtype{\M}{\tau}}}
  }{\ruleBArrowI}
  \quad
  \derivable{\Phi_{u}}{\sequB{\Delta}{\assign{u}{\M}}}{\SysBang}
}{
  \derivable{\Phi}{\sequB{\Gamma}{\assign{\termapp{(\termabs{x}{s})}{u}}{\tau}}}{\SysBang}
}{\ruleBArrowE}
      $$ and we conclude with $$
\Rule{
  \derivable{\Phi_{s}}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}
  \quad
  \derivable{\Phi_{u}}{\sequB{\Delta}{\assign{u}{\M}}}{\SysBang}
}{
  \derivable{\Phi'}{\sequB{\Gamma}{\assign{\termsubs{x}{u}{s}}{\tau}}}{\SysBang}
}{\ruleBESubs} $$
      Note that $\size{\Phi} = \size{\Phi'} + 1$.
 
      \item $\ctxt{L} = \termsubs{y}{r}{\ctxt{L'}}$. Then $\Gamma =
      \ctxtsum{(\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta'}{})}{\Delta}{}$
      s.t. $(\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta'}{})(x) = \M$ and
      $\Gamma'(y) = \M'$ and
      $$\kern-5em
\prooftree
  \Rule{
    \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{\functtype{\M}{\tau}}}}{\SysBang}
    \quad
    \derivable{\Phi_{r}}{\sequB{\Delta'}{\assign{r}{\M'}}}{\SysBang}
  }{
    \sequB{\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta'}{}}{\assign{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{\functtype{\M}{\tau}}}
  }{\ruleBESubs}
  \quad
  \derivable{\Phi_{u}}{\sequB{\Delta}{\assign{u}{\M}}}{\SysBang}
\justifies
  \derivable{\Phi}{\sequB{\Gamma}{\assign{\termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{s}}}{u}}{\tau}}}{\SysBang}
\using
  \ruleBArrowE
\endprooftree
      $$ Thus, we build $$
\Rule{
  \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{\functtype{\M}{\tau}}}}{\SysBang}
  \quad
  \derivable{\Phi_{u}}{\sequB{\Delta}{\assign{u}{\M}}}{\SysBang}
}{
  \derivable{\Psi}{\sequB{\ctxtsum{\Gamma'}{\Delta}{}}{\assign{\termapp{\ctxtapp{\ctxt{L'}}{\termabs{x}{s}}}{u}}{\tau}}}{\SysBang}
}{\ruleBArrowE}
      $$ and by \ih there exists $\derivable{\Psi'}{\sequB{\ctxtsum{\Gamma'}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L'}}{\termsubs{x}{u}{s}}}{\tau}}}{\SysBang}$. Then, we conclude with $$
\Rule{
  \derivable{\Psi'}{\sequB{\ctxtsum{\Gamma'}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L'}}{\termsubs{x}{u}{s}}}{\tau}}}{\SysBang}
  \quad
  \derivable{\Phi_{r}}{\sequB{\Delta'}{\assign{r}{\M'}}}{\SysBang}
}{
  \derivable{\Phi'}{\sequB{\ctxtsum{(\ctxtsum{(\ctxtres{\Gamma'}{y}{})}{\Delta'}{})}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L}}{\termsubs{x}{u}{s}}}{\tau}}}{\SysBang}
}{\ruleBESubs} $$
      since we may assume that $y \notin \dom{\Delta}$. Notice that $\size{\Phi} = \size{\Psi} + \size{\Phi_{r}} + 1 > \size{\Psi'} + \size{\Phi_{r}} + 1 = \size{\Phi'}$.
    \end{itemize}
    
    \item Rule $\sBang$. Then $t = \termsubs{x}{\ctxtapp{\ctxt{L}}{\termbang{u}}}{s}$
    and $t' = \ctxtapp{\ctxt{L}}{\substitute{x}{u}{s}}$. We proceed by induction
    on $\ctxt{L}$.
    \begin{itemize}
      \item $\ctxt{L} = \Box$. Then $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta_i}{i \in I}$
      s.t. $\Gamma'(x) = \intertype{\sigma}{i \in I}$ and $$
\prooftree
  \derivable{\Phi_{s}}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}
  \quad
  \Rule{
    \many{\derivable{\Phi^{i}_{u}}{\sequB{\Delta_i}{\assign{u}{\sigma_i}}}{\SysBang}}{i \in I}
  }{
    \sequB{\ctxtsum{}{\Delta_i}{i \in I}}{\assign{\termbang{u}}{\intertype{\sigma}{i \in I}}}
  }{\ruleBBang}
\justifies
  \derivable{\Phi}{\sequB{\Gamma}{\assign{\termsubs{x}{\termbang{u}}{s}}{\tau}}}{\SysBang}
\using
  \ruleBESubs
\endprooftree $$
      Thus, we conclude directly by Lem.~\ref{l:substitution-bang} with $\Phi_{s}$ and
      $\many{\Phi^{i}_{u}}{i \in I}$. Notice that $\size{\Phi} = \size{\Phi_s} +_{i \in I} \size{\Phi^i_u} + 2$, while $\size{\Phi'} = \size{\Phi_s} +_{i \in I} \size{\Phi^i_u} - |I|$.
      
      \item $\ctxt{L} = \termsubs{y}{r}{\ctxt{L'}}$. Then $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\ctxtsum{(\ctxtres{\Delta}{y}{})}{\Delta'}{}}{}$ with $\Gamma'(x) = \M$, $\Delta(y) = \M'$ and $$
\prooftree
  \derivable{\Phi_{s}}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}
  \quad
  \Rule{
    \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Delta}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{u}}}{\M}}}{\SysBang}
    \quad
    \derivable{\Phi_{r}}{\sequB{\Delta'}{\assign{r}{\M'}}}{\SysBang}
  }{
  \sequB{\ctxtsum{(\ctxtres{\Delta}{y}{})}{\Delta'}{}}{\assign{\ctxtapp{\termsubs{y}{r}{\ctxt{L'}}}{\termbang{u}}}{\M}}
  }{\ruleBESubs}
\justifies
  \derivable{\Phi}{\sequB{\Gamma}{\assign{\termsubs{x}{
  \ctxtapp{\ctxt{L}}{\termbang{u}}
  }{s}}{\tau}}}{\SysBang}
\using
  \ruleBESubs
\endprooftree
      $$ Thus, we build $$
\Rule{
  \derivable{\Phi_{s}}{\sequB{\Gamma'}{\assign{s}{\tau}}}{\SysBang}
  \quad
  \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Delta}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{u}}}{\M}}}{\SysBang}
}{
  \derivable{\Psi}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}}{\assign{\termsubs{x}{
  \ctxtapp{\ctxt{L'}}{\termbang{u}}
  }{s}}{\tau}}}{\SysBang}
}{\ruleBESubs}
      $$ and by the \ih there exists
      $\derivable{\Psi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L'}}{\substitute{x}{u}{s}}}{\tau}}}{\SysBang}$.
      Then, we conclude with $$
\Rule{
  \derivable{\Psi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}}{\assign{\ctxtapp{\ctxt{L'}}{\substitute{x}{u}{s}}}{\tau}}}{\SysBang}
  \quad
  \derivable{\Phi_{r}}{\sequB{\Delta'}{\assign{r}{\M'}}}{\SysBang}
}{
  \derivable{\Phi'}{\sequB{\ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\ctxtsum{(\ctxtres{\Delta}{y}{})}{\Delta'}{}}{}}{\assign{\ctxtapp{\ctxt{L}}{\substitute{x}{u}{s}}}{\tau}}}{\SysBang}
}{\ruleBESubs} $$
      since we may assume that $y \notin \dom{\Gamma'}$. Notice that $\size{\Phi} = \size{\Psi} + \size{\Phi_{r}} + 1 > \size{\Psi'} + \size{\Phi_{r}} + 1 = \size{\Phi'}$.
    \end{itemize}
    
    \item Rule $\dBang$. Then $t = \termder{\ctxtapp{\ctxt{L}}{\termbang{s}}}$
    and $t' = \ctxtapp{\ctxt{L}}{s}$. We proceed by induction on $\ctxt{L}$.
    \begin{itemize}
      \item $\ctxt{L} = \Box$. This case is immediate since $$
\prooftree
  \Rule{
    \derivable{\Phi'}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}
  }{
    \sequB{\Gamma}{\assign{\termbang{s}}{\intertype{\tau}{}}}
  }{\ruleBBang}
\justifies
  \derivable{\Phi}{\sequB{\Gamma}{\assign{\termder{\termbang{s}}}{\tau}}}{\SysBang}
\using
  \ruleBDer
\endprooftree $$
      \item $\ctxt{L} = \termsubs{y}{r}{\ctxt{L'}}$. Then $\Gamma =
      \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$ with $\Gamma'(x) = \M$ and $$
\prooftree
  \Rule{
    \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{s}}}{\intertype{\tau}{}}}}{\SysBang}
    \quad
    \derivable{\Phi_{r}}{\sequB{\Delta}{\assign{r}{\M}}}{\SysBang}
  }{
    \sequB{\Gamma}{\assign{\ctxtapp{\ctxt{L}}{\termbang{s}}}{\intertype{\tau}{}}}
  }{\ruleBESubs}
\justifies
  \derivable{\Phi}{\sequB{\Gamma}{\assign{\termder{\ctxtapp{\ctxt{L}}{\termbang{s}}}}{\tau}}}{\SysBang}
\using
  \ruleBDer
\endprooftree
      $$ Thus, we build $$
\Rule{
  \derivable{\Phi_{\ctxt{L'}}}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{\termbang{s}}}{\intertype{\tau}{}}}}{\SysBang}
}{
  \derivable{\Psi}{\sequB{\Gamma'}{\assign{\termder{\ctxtapp{\ctxt{L'}}{\termbang{s}}}}{\tau}}}{\SysBang}
}{\ruleBDer}
      $$ and by the \ih there exists
      $\derivable{\Psi'}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{s}}{\tau}}}{\SysBang}$.
      Hence we conclude $$
\Rule{
  \derivable{\Psi'}{\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L'}}{s}}{\tau}}}{\SysBang}
  \quad
  \derivable{\Phi_{r}}{\sequB{\Delta}{\assign{r}{\M}}}{\SysBang}
}{
  \derivable{\Phi'}{\sequB{\Gamma}{\assign{\ctxtapp{\ctxt{L}}{s}}{\tau}}}{\SysBang}  
}{\ruleBESubs} $$
      Notice that $\size{\Phi} = \size{\Psi} + \size{\Phi_{r}} + 1 >
      \size{\Psi'} + \size{\Phi_{r}} + 1 = \size{\Phi'}$.
    \end{itemize}
  \end{itemize}
  
  \item All the inductive cases for $\ctxt{S}$ are straightforward by the \ih
\end{itemize}
\end{proof}


==> proofs/bang/substitution-tight.tex <==
\begin{proof}
Straightforward induction on $\Phi_t$. The detailed proof of few chosen cases
follow. Suppose that the last rule of  $\Phi_t$ is:
\begin{itemize}
  \item $\ruleBDAxiom$. Then $t = y$ and  $\Gamma = y:\intertype{\tau}{}$. If
  $x \neq y$ then $I=\emptyset$, and the required typing is $\Phi_{t}$. If $x =
  y$ then $I$ is a singleton $\{*\}$ and the required typing is $\Phi^{*}_{u}$.
  The counters are as expected since $\cmult = \cexp = \csize = 0$.
  
  \item $\ruleBDApp$. Then $t = \termapp{t_1}{t_2}$ and there exist two type
  derivations
  $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1;\assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\functtype{\M}{\tau}}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$
  and
  $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2; \assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\typeneutral}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
  such that $\Gamma = \ctxtsum{\Gamma_1}{\Gamma_2}{}$, $I = I_1 \uplus I_2$,
  $\cmult = \cmult_1 + \cmult_2 + 1$, $\cexp = \cexp_1 + \cexp_2$,
  $\csize =
  \csize_1 + \csize_2$, and $\M$ is tight. The \ih provides the typings 
  $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}}{\assign{\substitute{x}{u}{t_1}}{\functtype{\M}{\tau}}}{\cmult_1 +_{\iI_1}{\cmult_i}}{\cexp_1 +_{\iI_1}{\cexp_i}}{\csize_1 +_{\iI_1}{\csize_i}}}{\SysTight}$
  and
  $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{\assign{\substitute{x}{u}{t_2}}{\typeneutral }}{\cmult_2 +_{\iI_2}{\cmult_i}}{\cexp_2 +_{\iI_2}{\cexp_i}}{\csize_2 +_{\iI_2}{\csize_i}}}{\SysTight}$.
  The required typing is obtained by applying the rule $\ruleBDApp$ to these,
  using the fact that $\M$ is tight. The counters are as expected. % using the \ih
  
  \item $\ruleBDESubs$. Then $ t = \termsubs{y}{t_2}{t_1}$, and we have
  $\derivable{\Phi_{t_1}}{\sequT{\Gamma_1; \assign{x}{\intertype{\sigma_i}{i \in I_1}}}{\assign{t_1}{\tau}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTight}$
  and
  $\derivable{\Phi_{t_2}}{\sequT{\Gamma_2; \assign{x}{\intertype{\sigma_i}{i \in I_2}}}{\assign{t_2}{\Gamma_1(y)}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTight}$
  such that $\Gamma = \ctxtsum{(\ctxtres{\Gamma_1}{y}{})}{\Gamma_2}{}$, $I = I_1
  \uplus I_2$, $\cmult = \cmult_1 + \cmult_2$, $\cexp = \cexp_1 + \cexp_2$,
  $\csize = \csize_1 + \csize_2$. The  \ih provides the typings 
  $\derivable{\Phi_{\substitute{x}{u}{t_1}}}{\sequT{\ctxtsum{\Gamma_1}{\Delta_i}{i \in I_1}}{\assign{\substitute{x}{u}{t_1}}{\tau}}{\cmult_1 +_{\iI_1}{\cmult_i}}{\cexp_1 +_{\iI_1}{\cexp_i}}{\csize_1 +_{\iI_1}{\csize_i}}}{\SysTight}$
  and 
  $\derivable{\Phi_{\substitute{x}{u}{t_2}}}{\sequT{\ctxtsum{\Gamma_2}{\Delta_i}{i \in I_2}}{\assign{\substitute{x}{u}{t_2}}{ \Gamma_1(y)}}{\cmult_2 +_{\iI_2}{\cmult_i}}{\cexp_2 +_{\iI_2}{\cexp_i}}{\csize_2 +_{\iI_2}{\csize_i}}}{\SysTight}$
  The required typing is obtained by  applying the rule $\ruleBDESubs$ to
  these. The counters are as expected. % using the \ih
\end{itemize}
\end{proof}


==> proofs/bang/substitution.tex <==


\begin{proof}
Straightforward induction on $\Phi_t$. 
\end{proof}



==> proofs/bang/tight-size.tex <==
\begin{proof}
By induction on $\Phi$.
\begin{itemize}
  \item $\ruleBDAxiom$. Then $t = x$ and $\csize = 0 = \wsize{t}$.
  
  \item $\ruleBTArrowE$. Then $t = \termapp{r}{u}$, $\sigma = \typeneutral$,
  $\Gamma = \ctxtsum{\Gamma'}{\Delta}{}$, $\csize = \csize' + \csize'' + 1$,
  $\derivable{\Phi_r}{\sequT{\Gamma'}{\assign{r}{\typeneutral}}{0}{0}{\csize'}}{\SysTight}$,
  $\derivable{\Phi_u}{\sequT{\Delta}{\assign{u}{\overline{\typeabs}}}{0}{0}{\csize''}}{\SysTight}$.
  Then, $\Gamma'$ and $\Delta$ are both tight, hence the \ih gives $\csize' =
  \wsize{r}$ and $\csize'' = \wsize{u}$. Hence, $\csize = \wsize{r} +
  \wsize{u} + 1 = \wsize{t}$.
  
  \item $\ruleBDApp$. This case does not apply since it concludes
  with $\cmult > 0$.
  
  \item $\ruleBDArrowE$. This case does not apply since it concludes
  with $\cmult > 0$.
  
  \item $\ruleBTArrowI$. Then $t = \termabs{x}{u}$, $\sigma = \typeabs$, $\Gamma
  = \ctxtres{\Gamma'}{x}{}$, $\csize = \csize' + 1$,
  $\derivable{\Phi_u}{\sequT{\Gamma'}{\assign{u}{\typetight}}{0}{0}{\csize'}}{\SysTight}$
  and $\ptight{\Gamma'(x)}$. Since $\Gamma$ is tight and $\ptight{\Gamma'(x)}$,
  $\Gamma'$ is tight as well. Then, by \ih $\csize' = \wsize{u}$, which implies
  $\csize = \wsize{u} + 1 = \wsize{t}$.
  
  \item $\ruleBDArrowI$. Then $\sigma = \functtype{\M}{\tau}$ which
  contradicts the hypothesis of $\Phi$ being tight. Hence, this case does not
  apply.
  
  \item $\ruleBTBang$. Then $t = \termbang{u}$ and $\csize = 0 = \wsize{t}$.
  
  \item $\ruleBDBang$. This case does not apply since it concludes with
  $\cexp > 0$.
  
  \item $\ruleBTDer$. Then $t = \termder{u}$, $\sigma = \typeneutral$,
  $\csize = \csize' + 1$ and
  $\derivable{\Phi_u}{\sequT{\Gamma}{\assign{u}{\typeneutral}}{0}{0}{\csize'}}{\SysTight}$.
  By \ih $\csize' = \wsize{u}$, which implies $\csize = \wsize{u} + 1 =
  \wsize{t}$.
  
  \item $\ruleBDDer$. Then $t = \termder{u}$ and
  $\derivable{\Phi_u}{\sequT{\Gamma}{\assign{u}{\intertype{\sigma}{}}}{0}{0}{\csize}}{\SysTight}$.
  Then, Lem.~\ref{l:tight-spreading-czero} on $\Phi_u$ gives
  $\intertype{\sigma}{} \in \typetight$ which is clearly a contradiction. Thus,
  this case does not apply.
  
  \item $\ruleBTESubs$. Then $t = \termsubs{x}{u}{r}$, $\Gamma =
    \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$,
    $\csize = \csize' + \csize''$,
  $\derivable{\Phi_r}{\sequT{\Gamma'}{\assign{r}{\sigma}}{0}{0}{\csize'}}{\SysTight}$,
  $\derivable{\Phi_u}{\sequT{\Delta}{\assign{u}{\typeneutral}}{0}{0}{\csize''}}{\SysTight}$
  and $\ptight{\Gamma'(x)}$. Since $\Gamma$ is tight and $\ptight{\Gamma'(x)}$,
  then $\Gamma'$ and $\Delta$ are both tight as well. Thus, \ih gives
  $\csize' = \wsize{r}$ and $\csize'' = \wsize{u}$. Then,
  $\csize = \wsize{r} +
  \wsize{u}  = \wsize{t}$. 
  
  \item $\ruleBDESubs$. Then $t = \termsubs{x}{u}{r}$, $\csize = \csize' +
  \csize''$ and $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$ tight
  such that, in particular,
  $\derivable{\Phi_u}{\sequT{\Delta}{\assign{u}{\Gamma'(x)}}{0}{0}{\csize''}}{\SysTight}$
  with $\Delta$ tight. By Lem.~\ref{l:tight-spreading-czero} on $\Phi_u$,
  $\Gamma'(x) \in \typetight$ which leads to a contradiction, since
  $\Gamma'(x)$ is a multiset type by definition. Hence, this case does not
  apply.
\end{itemize}
\end{proof}


==> proofs/bang/tight-spreading-czero.tex <==
\begin{proof}
By induction on $\Phi$. Note that the statement trivially holds for the
rules $\ruleBTArrowE$, $\ruleBTArrowI$, $\ruleBTBang$, $\ruleBTDer$, $\ruleBTESubs$,
$\ruleBDApp$ in Fig.~\ref{fig:typingSchemesTight} since all of them conclude
with $\sigma \in \typetight$. We proceed by analysing the other rules in
Fig.~\ref{fig:typingSchemesTight}.
\begin{itemize}
  \item $\ruleBDAxiom$. Then $t = x$ and $\Gamma =
  \assign{x}{\intertype{\sigma}{}}$ tight which implies $\sigma \in \typetight$.
    
  \item $\ruleBDArrowE$. This case does not apply since it concludes with
  $\cmult > 0$.
  
  \item $\ruleBDArrowI$. This case does not apply since it concludes with an
  arrow type.
  
  \item $\ruleBDBang$. This case does not apply since it concludes with
  $\cexp > 0$.
  
  \item $\ruleBDDer$. Then $t = \termder{u}$ and
  $\sequT{\Gamma}{\assign{u}{\intertype{\sigma}{}}}{0}{0}{\csize}$ is
  derivable. Then, the \ih gives $\intertype{\sigma}{} \in \typetight$
  which is clearly a contradiction. Thus, this case does not apply either.
  
  \item $\ruleBDESubs$. Then $t = \termsubs{x}{u}{r}$, $\csize = \csize' +
  \csize''$ and $\Gamma = \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$ tight
  such that, in particular
  $\sequT{\Delta}{\assign{u}{\Gamma(x)}}{0}{0}{\csize''}$ with $\Delta$
  tight. The \ih gives $\Gamma(x) \in \typetight$ which leads to a
  contradiction since it is a multiset type. Hence, this case does not apply.
\end{itemize}
\end{proof}


==> proofs/bang/tight-spreading-neutral.tex <==
\begin{proof}
By induction on $t$, considering that $\pntrl{t}$ holds.
\begin{itemize}
  \item $t = x$. Then, $\Phi$ ends with rule $\ruleBDAxiom$ and $\Gamma =
  \assign{x}{\intertype{\sigma}{}}$ tight implies $\sigma \in \typetight$.
  
  \item $t = \termapp{r}{u}$. By definition of $\pntrl{t}$, $\pnabs{r}$ and
  $\pnrml{u}$ hold. Moreover, $\neg\pbang{r}$ by
  Lem.~\ref{l:clashes-do-not-type}. Then, by Rem.~\ref{r:normal}, it is
  necessarily the case that $\pnbang{r}$ holds, and hence $\pntrl{r}$ as
  well. There are three cases for $\Phi$:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTArrowE$, then $\sigma =
    \typeneutral$ and the statement trivially holds.
    
    \item if $\Phi$ ends with rule $\ruleBDApp$, then $\sigma \in \typetight$
    and the statement  trivially holds.
    
    \item if $\Phi$ ends with rule $\ruleBDArrowE$, then $\Gamma =
    \ctxtsum{\Gamma'}{\Delta}{}$, $\cmult = \cmult' + \cmult'' + 1$, $\cexp =
    \cexp' + \cexp''$, $\csize = \csize' + \csize''$ and, in particular,
    $\derivable{\Phi_r}{\sequT{\Gamma'}{\assign{r}{\functtype{\M}{\tau}}}{\cmult'}{\cexp'}{\csize'}}{\SysTight}$.
    Then, $\pntrl{r}$ gives $\functtype{\M}{\tau} \in \typetight$ by \ih
    This is clearly a contradiction. Hence, this case does not apply.
  \end{enumerate}
  
  \item $t = \termder{u}$. By definition of $\pntrl{t}$, $\pnbang{u}$ holds.
  Moreover, $\neg\pabs{u}$ by Lem.~\ref{l:clashes-do-not-type}. Then, by
  Rem.~\ref{r:normal}, it is necessarily the case that $\pnabs{u}$ holds,
  and hence $\pntrl{u}$ as well. Then, there are two cases for
  $\Phi$:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTDer$, then $\sigma = \typeneutral$
    and the statement  trivially holds.
    
    \item if $\Phi$ ends with rule $\ruleBDDer$, then
    $\derivable{\Phi_u}{\sequT{\Gamma}{\assign{u}{\intertype{\sigma}{}}}{\cmult}{\cexp}{\csize}}{\SysTight}$.
    Therefore, $\pntrl{u}$ gives $\intertype{\sigma}{} \in \typetight$ by \ih
    This is clearly a contradiction. Hence, this case does not apply.
  \end{enumerate}
  
  \item $t = \termsubs{x}{u}{r}$. By definition of $\pntrl{t}$, $\pnbang{u}$
  holds. Moreover, $\neg\pabs{u}$ by Lem.~\ref{l:clashes-do-not-type}. Then,
  by Rem.~\ref{r:normal}, it is necessarily the case that $\pnabs{u}$ holds,
  and hence $\pntrl{u}$ as well. Then, there are two cases for $\Phi$:
  \begin{enumerate}
    \item if $\Phi$ ends with rule $\ruleBTESubs$, then $\sigma \in
    \typetight$ and the statement trivially holds.
    
    \item if $\Phi$ ends with rule $\ruleBDESubs$, $\Gamma =
    \ctxtsum{\ctxtres{\Gamma'}{x}{}}{\Delta}{}$, $\cmult = \cmult' +
    \cmult''$, $\cexp = \cexp' + \cexp''$, $\csize = \csize' + \csize''$ and,
    in particular,
    $\derivable{\Phi_u}{\sequT{\Delta}{\assign{u}{\Gamma'(x)}}{\cmult''}{\cexp''}{\csize''}}{\SysTight}$.
    Then, $\pntrl{u}$ gives $\Gamma'(x) \in \typetight$ by \ih
    This leads to a contradiction, since $\Gamma'(x)$ is a multiset type by
    definition. Hence, this case does not apply.
  \end{enumerate}
\end{itemize}
\end{proof}


==> proofs/cbn-cbv-normalisation.tex <==
\begin{proof}
Sec.~\ref{s:technical-name} and~\ref{s:technical-value} below show the two
statements separately as Thm.~\ref{t:normalisation-name} and
Thm.~\ref{t:normalisation-value} respectively.
\end{proof}



==> proofs/cbn-cbv-preservation.tex <==
\begin{proof}\mbox{} 
\begin{enumerate}
  \item By Lem.~\ref{l:normal-forms-cbn-cbv} and Prop.~\ref{prop:normal} it
  is sufficient to prove that $t \in \CBNNF$ implies $\pnrml{\cbnterm{t}}$. This is
  done by simultaneously showing the following points:
  \begin{enumerate}
    \item\label{l:preservation-cbn-ne} If $t \in \HCBNNF$, then $\pntrl{\cbnterm{t}}$.
    \item\label{l:preservation-cbn-no} If $t \in \CBNNF$, then $\pnrml{\cbnterm{t}}$.
  \end{enumerate}
  
  \begin{itemize}
    \item If $t = x \in \HCBNNF$, then $\cbnterm{x} = x$ and thus $\pntrl{x}$
    holds.
    
    \item If $t = \termapp{s}{u} \in \HCBNNF$ comes from $s \in \HCBNNF$, then
    the \ih (\ref{l:preservation-cbn-ne}) gives $\pntrl{\cbnterm{s}}$ and hence
    $\pnabs{\cbnterm{s}}$. Moreover
    $\pnabs{\termbang{\cbnterm{u}}}$ also holds, which implies
    $\pnrml{\termbang{\cbnterm{u}}}$. We can then conclude
    $\pntrl{\termapp{\cbnterm{s}}{\termbang{\cbnterm{u}}}}$, \ie
    $\pntrl{\cbnterm{(\termapp{s}{u})}}$.
    
    \item If $t \in \CBNNF$ comes from $t \in \HCBNNF$, then $\pntrl{\cbnterm{t}}$
    holds by the previous point, which gives $\pnrml{\cbnterm{t}}$.
    
    \item If $t = \termabs{x}{u} \in \CBNNF$ comes from $u \in \CBNNF$, then
    the \ih (\ref{l:preservation-cbn-no}) gives $\pnrml{\cbnterm{u}}$, which implies
    $\pnbang{\termabs{x}{\cbnterm{u}}}$, thus giving
    $\pnrml{\termabs{x}{\cbnterm{u}}}$. We conclude since $\cbnterm{(\termabs{x}{u})} =
    \termabs{x}{\cbnterm{u}}$.
  \end{itemize}
  
  \item By Lem.~\ref{l:normal-forms-cbn-cbv} and Prop.~\ref{prop:normal} it
  is sufficient to prove that $t \in \CBVNF$ implies $\pnrml{\cbvterm{t}}$. This is
  done by simultaneously showing the following points:
  \begin{enumerate}
    \item\label{l:preservation-cbv-vr} If $t \in \VarHCBVNF$, then $\pnabs{\cbvterm{t}}$.
    \item\label{l:preservation-cbv-ne} If $t \in \HCBVNF$, then $\pntrl{\cbvterm{t}}$.
    \item\label{l:preservation-cbv-no} If $t \in \CBVNF$, then $\pnrml{\cbvterm{t}}$.
  \end{enumerate}
  
  \begin{itemize}
    \item If $t = x \in \VarHCBVNF$, then $\cbvterm{x} = \termbang{x}$ and
    $\pnabs{\termbang{x}}$.
    
    \item If $t = \termsubs{x}{u}{s} \in \VarHCBVNF$ comes from $s \in
    \VarHCBVNF$ and $u \in \HCBVNF$, then the \ih (\ref{l:preservation-cbv-vr}) gives $\pnabs{\cbvterm{s}}$ and
    $\pntrl{\cbvterm{u}}$ which in turn implies $\pnbang{\cbvterm{u}}$. Hence, it
    allows to conclude $\pnabs{\termsubs{x}{\cbvterm{u}}{\cbvterm{s}}}$.
    
    \item If $t = \termapp{s}{u} \in \HCBVNF$ comes from $s \in \VarHCBVNF$ and
    $u \in \CBVNF$. It is immediate to see that $\cbvterm{s} =
    \ctxtapp{\ctxt{L}}{\termbang{x}}$ for some variable $x$. Thus, $\cbvterm{t} =
    \termapp{\ctxtapp{\ctxt{L}}{x}}{\cbvterm{u}}$. Moreover, by \ih (\ref{l:preservation-cbv-vr})
    $\pnabs{\cbvterm{s}}$ holds, which implies $\pnbang{r}$ for all $\exsubs{y}{r}$
    in $\ctxt{L}$. Thus, $\pntrl{\ctxtapp{\ctxt{L}}{x}}$ holds.
    This implies $\pnabs{\ctxtapp{\ctxt{L}}{x}}$, by definition. Also, the \ih
    (\ref{l:preservation-cbv-no}) on $u \in \CBVNF$ gives $\pnrml{\cbvterm{u}}$. Hence, we conclude
    $\pntrl{\cbvterm{t}}$.

    \item If $t = \termapp{s}{u} \in \HCBVNF$ comes from $s \in \HCBVNF$ and
    $u \in \CBVNF$. By \ih (\ref{l:preservation-cbv-ne}) $\pntrl{\cbvterm{s}}$ holds. In particular it implies
    $\pnbang{\cbvterm{s}}$ (\ie $\neg\pbang{\cbvterm{s}}$). Hence, $\cbvterm{t} =
    \termapp{\termder{(\cbvterm{s})}}{\cbvterm{u}}$ and $\pntrl{\termder{(\cbvterm{s})}}$.
    Moreover, the latter implies $\pnabs{\termder{(\cbvterm{s})}}$, by definition.
    Also, the \ih (\ref{l:preservation-cbv-no}) on $u \in \CBVNF$ gives $\pnrml{\cbvterm{u}}$. Thus, we conclude
    $\pntrl{\cbvterm{t}}$.
    
    \item If $t = \termsubs{x}{u}{s} \in \HCBVNF$ comes from $s \in \HCBVNF$
    and $u \in \HCBVNF$, then the \ih (\ref{l:preservation-cbv-ne}) gives $\pntrl{\cbvterm{s}}$ and
    $\pntrl{\cbvterm{u}}$ which in turn implies $\pnbang{\cbvterm{u}}$. Hence, it
    allows to conclude $\pntrl{\termsubs{x}{\cbvterm{u}}{\cbvterm{s}}}$.
    
    \item If $t = \termabs{x}{s} \in \CBVNF$, then $\cbvterm{t} =
    \termbang{\termabs{x}{\cbvterm{s}}}$. Thus, $\pnabs{\cbvterm{t}}$ holds and we
    conclude $\pnrml{\cbvterm{t}}$.
    
    \item If $t \in \CBVNF$ comes from $t \in \VarHCBVNF$. Then,
    item (\ref{l:preservation-cbv-vr}) gives
    $\pnabs{\cbvterm{t}}$ which implies $\pnrml{\cbvterm{t}}$ by definition.

    \item If $t \in \CBVNF$ comes from $t \in \HCBVNF$. Then, item
    (\ref{l:preservation-cbv-ne}) gives $\pntrl{\cbvterm{t}}$ which
    implies $\pnrml{\cbvterm{t}}$.
    
    \item If $t = \termsubs{x}{u}{s} \in \CBVNF$ comes from $s \in \CBVNF$
    and $u \in \HCBVNF$, then the \ih (\ref{l:preservation-cbv-no}) and
    (\ref{l:preservation-cbv-ne}) gives $\pnrml{\cbvterm{s}}$ and
    $\pntrl{\cbvterm{u}}$ which in turn implies $\pnbang{\cbvterm{u}}$. Hence, it
    allows to conclude $\pnrml{\termsubs{x}{\cbvterm{u}}{\cbvterm{s}}}$.
  \end{itemize}
\end{enumerate}
\end{proof}



==> proofs/cbn-cbv-reduction.tex <==
\begin{proof}
Both proofs are by induction on the reduction relations.
\begin{enumerate}
  \item Case $t  \rewrite{\callbyname} s$.
  \begin{itemize}
    \item $t = \termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{r}}}{u} \rrule{\dBeta}
    \ctxtapp{\ctxt{L}}{\termsubs{x}{u}{r}} = s$. Then, $$\cbnterm{t} =
    \termapp{\ctxtapp{\cbnterm{\ctxt{L}}}{\termabs{x}{\cbnterm{r}}}}{\termbang{\cbnterm{u}}}
    \rewrite{\dBeta}
    \ctxtapp{\cbnterm{\ctxt{L}}}{\termsubs{x}{\termbang{\cbnterm{u}}}{\cbnterm{r}}} =
    \cbnterm{s}$$
    
    \item $t = \termsubs{x}{u}{r} \rrule{\sTerm} \substitute{x}{u}{r} = s$.
    Then, $$\cbnterm{t} = \termsubs{x}{\termbang{\cbnterm{u}}}{\cbnterm{r}}
    \rewrite{\sBang} \substitute{x}{\cbnterm{u}}{\cbnterm{r}}
    =_{L.\ref{l:substitution-cbn-cbv}} \cbnterm{s}$$
    
    \item $t = \termapp{r}{u} \rewrite{\callbyname} \termapp{r'}{u} = s$, or
    $t = \termabs{x}{r} \rewrite{\callbyname} \termabs{x}{r'} = s$, or $t =
    \termsubs{x}{u}{r} \rewrite{\callbyname} \termsubs{x}{u}{r'} = s$, where
    $r \rewrite{\callbyname} r'$. Then, we easily conclude by the \ih
  \end{itemize}
  
  \item Case $t \rewrite{\callbyvalue} s$.
  \begin{itemize}
    \item $t = \termapp{\ctxtapp{\ctxt{L}}{\termabs{x}{r}}}{u} \rrule{\dBeta}
    \ctxtapp{\ctxt{L}}{\termsubs{x}{u}{r}} = s$. Then, $$\cbvterm{t} =
    \termapp{\ctxtapp{\cbvterm{\ctxt{L}}}{\termabs{x}{\cbvterm{r}}}}{\cbvterm{u}}
    \rewrite{\dBeta} \ctxtapp{\cbvterm{\ctxt{L}}}{\cbvterm{r}\exsubs{x}{\cbvterm{u}}} =
    \cbvterm{s}$$
    
    \item $t = \termsubs{x}{\ctxtapp{\ctxt{L}}{v}}{r} \rrule{\sVal}
    \ctxtapp{\ctxt{L}}{\substitute{x}{v}{r}} = s$. Then, $$\cbvterm{t} =
    \termsubs{x}{\ctxtapp{\cbvterm{\ctxt{L}}}{\cbvterm{v}}}{\cbvterm{r}} \rewrite{\sBang}
    \ctxtapp{\cbvterm{\ctxt{L}}}{\substitute{x}{u}{\cbvterm{r}}}
    =_{L.\ref{l:substitution-cbn-cbv}} \cbvterm{s}$$ where $\cbvterm{v} =
    \termbang{u}$.
    
    \item $t = \termapp{r_0}{u} \rewrite{\callbyvalue} \termapp{r_1}{u} =
    s$ comes from $r_0 \rewrite{\callbyvalue} r_1$. The \ih gives $\cbvterm{r_0}
    \rewriten{\bangweak} \cbvterm{r_1}$. There are two cases:
    \begin{itemize}
      \item If $\cbvterm{r_0} = \ctxtapp{\ctxt{L}}{\termbang{r}}$, then $\cbvterm{t}
      = \termapp{\ctxtapp{\ctxt{L}}{r}}{\cbvterm{u}}$. The \ih implies in
      particular that $\cbvterm{r_1} = \ctxtapp{\ctxt{L}'}{\termbang{r'}}$, which
      implies in turn $\ctxtapp{\ctxt{L}}{r} \rewriten{\bangweak}
      \ctxtapp{\ctxt{L}'}{r'}$. We then have $\cbvterm{t} =
      \termapp{\ctxtapp{\ctxt{L}}{r}}{\cbvterm{u}} \rewriten{\bangweak}
      \termapp{\ctxtapp{\ctxt{L}'}{r'}}{\cbvterm{u}} = \cbvterm{s}$.
      
      \item Otherwise, $\cbvterm{t} = \termapp{\termder{(\cbvterm{r_0})}}{\cbvterm{u}}$.
      We have again two cases. 
      \begin{itemize}
        \item If $\cbvterm{r_1} = \ctxtapp{\ctxt{L}}{\termbang{r}}$, then $$\kern-5em
        \cbvterm{t} = \termapp{\termder{(\cbvterm{r_0})}}{\cbvterm{u}} \rewriten{\bangweak}
        \termapp{\termder{(\cbvterm{r_1})}}{\cbvterm{u}} =
        \termapp{\termder{(\ctxtapp{\ctxt{L}}{\termbang{r}})}}{\cbvterm{u}}
        \rewrite{\dBang} \termapp{\ctxtapp{\ctxt{L}}{r}}{\cbvterm{u}} = \cbvterm{s}$$
        
        \item Otherwise, the \ih allows us to conclude $$\cbvterm{t} =
        \termapp{\termder{(\cbvterm{r_0})}}{\cbvterm{u}} \rewriten{\bangweak} 
        \termapp{\termder{(\cbvterm{r_1})}}{\cbvterm{u}} = \cbvterm{s}$$
      \end{itemize}
    \end{itemize}
    
    \item $t = \termapp{r}{u} \rewrite{\callbyvalue} \termapp{r}{u'} =
    s$ comes from $u \rewrite{\callbyvalue} u'$. Then, there are two cases
    according to $\cbvterm{r}$ but the proof is easy using the \ih
    
    \item $t = \termsubs{x}{u}{r} \rewrite{\callbyvalue}
    \termsubs{x}{u}{r'} = s$ or $t = \termsubs{x}{r}{u}
    \rewrite{\callbyvalue} \termsubs{x}{r'}{u} = s$, where $r
    \rewrite{\callbyvalue} r'$. Then, we easily conclude by the \ih
  \end{itemize}
\end{enumerate}
\end{proof}



==> proofs/cbn-cbv-soundness-completeness.tex <==
\begin{proof}
\begin{enumerate}
  \item $\Rightarrow$) By induction on $t$.
  \begin{itemize}
    \item $t = x$. Then, $\Gamma = \assign{x}{\intertype{\sigma}{}}$
    and we conclude by rule $\ruleBAxiom$, since $\cbnterm{t} = x$.
    
    \item $t = \termapp{s}{u}$. Then, $\Gamma = \ctxtsum{\Gamma'}{\Delta_i}{i
    \in I}$, $\sequN{\Gamma'}{\assign{s}{\functtype{\intertype{\tau_i}{i \in
    I}}{\sigma}}}$ and $\many{\sequN{\Delta_i}{\assign{u}{\tau_i}}}{i \in I}$.
    By \ih $\sequB{\Gamma'}{\assign{\cbnterm{s}}{\functtype{\intertype{\tau_i}{i
    \in I}}{\sigma}}}$ and $\many{\sequB{\Delta_i}{\assign{\cbnterm{u}}{\tau_i}}}{i
    \in I}$. Moreover, by definition $\cbnterm{t} =
    \termapp{\cbnterm{s}}{\termbang{\cbnterm{u}}}$. Thus, we conclude by rules
    $\ruleBBang$ and $\ruleBArrowE$ \[
    \Rule{
      \sequB{\Gamma'}{\assign{\cbnterm{s}}{\functtype{\intertype{\tau_i}{i \in I}}{\sigma}}}
      \quad
      \Rule{
        \many{\sequB{\Delta_i}{\assign{\cbnterm{u}}{\tau_i}}}{i \in I}
      }{
        \sequ{\ctxtsum{}{\Delta_i}{i \in I}}{\assign{\termbang{\cbnterm{u}}}{\intertype{\tau_i}{i \in I}}}
      }{}
    }{
      \sequ{\ctxtsum{\Gamma'}{\Delta_i}{i \in I}}{\assign{\termapp{\cbnterm{s}}{\termbang{\cbnterm{u}}}}{\sigma}}
    }{} \]
    
    \item $t = \termabs{x}{s}$. Then, $\sigma = \functtype{\Gamma'(x)}{\tau}$,
    $\Gamma = \ctxtres{\Gamma'}{x}{}$ and $\sequN{\Gamma'}{\assign{s}{\tau}}$.
    By \ih $\sequB{\Gamma'}{\assign{\cbnterm{s}}{\tau}}$. Moreover, by definition
    $\cbnterm{t} = \termabs{x}{\cbnterm{s}}$, hence we conclude by rule $\ruleBArrowI$.
    
    \item $t = \termsubs{x}{u}{s}$. Then, $\Gamma =
    \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta_i}{i \in I}$,
    $\sequN{\Gamma'}{\assign{s}{\sigma}}$ and
    $\many{\sequN{\Delta_i}{\assign{u}{\tau_i}}}{i \in I}$ with $\Gamma'(x) =
    \intertype{\tau_i}{i \in I}$. By \ih
    $\sequB{\Gamma'}{\assign{\cbnterm{s}}{\sigma}}$ and
    $\many{\sequB{\Delta_i}{\assign{\cbnterm{u}}{\tau_i}}}{i \in I}$ hold. Finally,
    since $\cbnterm{t} = \termsubs{x}{\termbang{\cbnterm{u}}}{\cbnterm{s}}$, we conclude by
    rules $\ruleBBang$ and $\ruleBESubs$.
  \end{itemize}
  
  $\Leftarrow$) By induction on $t$.
  \begin{itemize}
    \item $t = x$. Then, $\cbnterm{x} = x$, $\Gamma =
    \assign{x}{\intertype{\sigma}{}}$ and the result is immediate using rule
    $\ruleNAxiom$.
    
    \item $t = \termapp{s}{u}$. Then, $\cbnterm{t} =
    \termapp{\cbnterm{s}}{\termbang{\cbnterm{u}}}$, $\Gamma =
    \ctxtsum{\Gamma'}{\Delta}{}$,
    $\sequB{\Gamma'}{\assign{\cbnterm{s}}{\functtype{\M}{\sigma}}}$ and
    $\sequB{\Delta}{\assign{\termbang{\cbnterm{u}}}{\M}}$. Moreover, by rule
    $\ruleBBang$, $\Delta = \ctxtsum{}{\Delta_i}{i \in I}$, $\M =
    \intertype{\tau_i}{i \in I}$ and
    $\many{\sequB{\Delta_i}{\assign{\cbnterm{u}}{\tau_i}}}{i \in I}$. The \ih 
    gives $\sequN{\Gamma'}{\assign{s}{\functtype{\intertype{\tau_i}{i \in
    I}}{\sigma}}}$ and $\many{\sequN{\Delta_i}{\assign{u}{\tau_i}}}{i \in I}$.
    Finally, we conclude by rule $\ruleNArrowE$.
    
    \item $t = \termabs{x}{s}$. Then $\cbnterm{t} = \termabs{x}{\cbnterm{s}}$, $\sigma
    = \functtype{\Gamma'(x)}{\tau}$, $\Gamma = \ctxtres{\Gamma'}{x}{}$ and
    $\sequB{\Gamma'}{\assign{\cbnterm{s}}{\tau}}$. The result follow immediately
    from the \ih using rule $\ruleNArrowI$.
    
    \item $t = \termsubs{x}{u}{s}$. Then, $\cbnterm{t} =
    \termsubs{x}{\termbang{\cbnterm{u}}}{\cbnterm{s}}$, $\Gamma =
    \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$,
    $\sequB{\Gamma'}{\assign{\cbnterm{s}}{\sigma}}$ and
    $\sequB{\Delta}{\assign{\termbang{\cbnterm{u}}}{\Gamma'(x)}}$. Moreover, by
    rule $\ruleBBang$, $\Delta = \ctxtsum{}{\Delta_i}{i \in I}$, $\Gamma'(x) =
    \intertype{\tau_i}{i \in I}$ and
    $\many{\sequB{\Delta_i}{\assign{\cbnterm{u}}{\tau_i}}}{i \in I}$. The \ih 
    gives $\sequN{\Gamma'}{\assign{s}{\sigma}}$ and $\many{\sequN{\Delta_i}{\assign{u}{\tau_i}}}{i \in I}$.
    Finally, we conclude by rule $\ruleNESubs$.
  \end{itemize}
  
  \item $\Rightarrow$) By induction on $t$.
  \begin{itemize}
    \item $t = x$. Then, $\sigma = \M$ and $\Gamma = \assign{x}{\M}$ where, by
    definition, $\M = \intertype{\tau_i}{i \in I}$. Moreover, by definition of
    the embedding, $\cbvterm{t} = \termbang{x}$. Thus, we conclude by rules
    $\ruleBAxiom$ and $\ruleBBang$ \[
    \Rule{
      \raisebox{0.5em}{$\Big(
        \raisebox{-0.25em}{\hspace{-1em}
          \Rule{}{\sequ{\assign{x}{\intertype{\tau_i}{}}}{\assign{x}{\tau_i}}}{}
        \hspace{-1em}}
      \Big)_{i \in I}$}
    }{
      \sequ{\assign{x}{\intertype{\tau_i}{i \in I}}}{\assign{\termbang{x}}{\intertype{\tau_i}{i \in I}}}
    }{} \]
    
    \item $t = \termapp{s}{u}$. Then, $\Gamma = \ctxtsum{\Gamma'}{\Delta}{}$, 
    $\sequV{\Gamma'}{\assign{s}{\intertype{\functtype{\M}{\sigma}}{}}}$ and
    $\sequV{\Delta}{\assign{u}{\M}}$. By \ih
    $\sequB{\Gamma'}{\assign{\cbvterm{s}}{\intertype{\functtype{\M}{\sigma}}{}}}$
    and $\sequB{\Delta}{\assign{\cbvterm{u}}{\M}}$. There are two cases:
    \begin{itemize}
      \item If $\cbvterm{s} = \ctxtapp{\ctxt{L}}{\termbang{r}}$, then $\cbvterm{t}
      = \termapp{\ctxtapp{\ctxt{L}}{r}}{\cbvterm{u}}$. From
      $\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L}}{\termbang{r}}}{\intertype{\functtype{\M}{\sigma}}{}}}$
      it is immediate to see,
      by induction on $\ctxt{L}$ using $\ruleBESubs$, that there exists $\Gamma''$ s.t.
      $\sequB{\Gamma''}{\assign{\termbang{r}}{\intertype{\functtype{\M}{\sigma}}{}}}$. Then,
      $\sequB{\Gamma''}{\assign{r}{\functtype{\M}{\sigma}}}$ holds from rule
      $\ruleBBang$. Moreover, by straighforward induction on $\ctxt{L}$ once
      again, we get
      $\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L}}{r}}{\functtype{\M}{\sigma}}}$.
      Finally, we conclude using  $\ruleBArrowE$ by using also
      $\sequB{\Delta}{\assign{\cbvterm{u}}{\M}}$.

      \item Otherwise, $\cbvterm{t} = \termapp{\termder{(\cbvterm{s})}}{\cbvterm{u}}$.
      Then, we resort to rules $\ruleBDer$ and $\ruleBArrowE$ to conclude \[
    \Rule{
      \Rule{
        \sequB{\Gamma'}{\assign{\cbvterm{s}}{\intertype{\functtype{\M}{\sigma}}{}}}
      }{
        \sequ{\Gamma'}{\assign{\termder{\cbvterm{s}}}{\functtype{\M}{\sigma}}}
      }{}
      \quad
      \sequB{\Delta}{\assign{\cbvterm{u}}{\M}}
    }{
      \sequ{\ctxtsum{\Gamma'}{\Delta}{}}{\assign{\termapp{\termder{(\cbvterm{s})}}{\cbvterm{u}}}{\sigma}}
    }{} \]
    \end{itemize}

    \item $t = \termabs{x}{s}$. Then $\sigma =
    \intertype{\functtype{\Gamma_i(x)}{\tau_i}}{i \in I}$, $\Gamma =
    \ctxtsum{}{\ctxtres{\Gamma_i}{x}{}}{i \in I}$ and
    $\many{\sequV{\Gamma_i}{\assign{s}{\tau_i}}}{i \in I}$. By \ih
    $\many{\sequB{\Gamma_i}{\assign{\cbvterm{s}}{\tau_i}}}{i \in I}$. Thus, we
    conclude with rules $\ruleBArrowI$ and $\ruleBBang$ since, by definition,
    $\cbvterm{t} = \termbang{\termabs{x}{\cbvterm{s}}}$ \[
    \Rule{
      \raisebox{1em}{$\Bigg(
        \raisebox{-0.75em}{\hspace{-1em}
          \Rule{
            \sequB{\Gamma_i}{\assign{\cbvterm{s}}{\tau_i}}
          }{
            \sequ{\ctxtres{\Gamma_i}{x}{}}{\assign{\termabs{x}{\cbvterm{s}}}{\functtype{\Gamma_i(x)}{\tau_i}}}
          }{}
        \hspace{-1em}}
      \Bigg)_{i \in I}$}
    }{
      \sequ{\ctxtsum{}{\ctxtres{\Gamma_i}{x}{}}{i \in I}}{\assign{\termbang{\termabs{x}{\cbvterm{s}}}}{\intertype{\functtype{\Gamma_i(x)}{\tau_i}}{i \in I}}}
    }{} \]
    
    \item $t = \termsubs{x}{u}{s}$. Then, $\Gamma =
    \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$,
    $\sequV{\Gamma'}{\assign{s}{\sigma}}$ and
    $\sequV{\Delta}{\assign{u}{\Gamma'(x)}}$. By \ih
    $\sequB{\Gamma'}{\assign{\cbvterm{s}}{\sigma}}$ and
    $\sequB{\Delta}{\assign{\cbvterm{u}}{\Gamma'(x)}}$ hold. Hence, since $\cbvterm{t} =
    \termsubs{x}{\cbvterm{u}}{\cbvterm{s}}$, we conclude by rule $\ruleBESubs$.
  \end{itemize}
  
  $\Leftarrow$) By induction on $t$.
  \begin{itemize}
    \item $t = x$. Then $\cbvterm{x} = \termbang{x}$, $\sigma =
    \intertype{\tau_i}{i \in I}$ and $\Gamma = \assign{x}{\intertype{\tau_i}{i
    \in I}}$. The result is immediate using rule $\ruleVAxiom$.
    
    \item $t = \termapp{s}{u}$. There are two cases to consider:
    \begin{itemize}
      \item If $\cbvterm{s} = \ctxtapp{\ctxt{L}}{\termbang{r}}$, then $\cbvterm{t} =
      \termapp{\ctxtapp{\ctxt{L}}{r}}{\cbvterm{u}}$. Then, $\Gamma =
      \ctxtsum{\Gamma'}{\Delta}{}$,
      $\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L}}{r}}{\functtype{\M}{\sigma}}}$
      and $\sequB{\Delta}{\assign{\cbvterm{u}}{\M}}$. Moreover, by induction on
      $\ctxt{L}$ using $\ruleBESubs$, it is immediate to see that there exists
      $\Gamma''$ s.t. $\sequB{\Gamma''}{\assign{r}{\functtype{\M}{\sigma}}}$. By
      rule $\ruleBBang$ we get
      $\sequB{\Gamma''}{\assign{\termbang{r}}{\intertype{\functtype{\M}{\sigma}}{}}}$
      and, by straightforward induction on $\ctxt{L}$ once again,
      $\sequB{\Gamma'}{\assign{\ctxtapp{\ctxt{L}}{\termbang{r}}}{\intertype{\functtype{\M}{\sigma}}{}}}$.
      Recall that the induction is on $t = \termapp{s}{u}$ and $\cbvterm{s}
      = \ctxtapp{\ctxt{L}}{\termbang{r}}$, hence by the \ih
      $\sequV{\Gamma'}{\assign{s}{\intertype{\functtype{\M}{\sigma}}{}}}$ and
      $\sequV{\Delta}{\assign{u}{\M}}$. Thus, we conclude by rule
      $\ruleVArrowE$.

      \item Otherwise, $\cbvterm{t} =
      \termapp{\termder{(\cbvterm{s})}}{\cbvterm{u}}$. We then have $\Gamma =
      \ctxtsum{\Gamma'}{\Delta}{}$,
      $\sequB{\Gamma'}{\assign{\termder{(\cbvterm{s})}}{\functtype{\M}{\sigma}}}$ and
      $\sequB{\Delta}{\assign{\cbvterm{u}}{\M}}$. Moreover, from rule $\ruleBDer$,
      we have
      $\sequB{\Gamma'}{\assign{\cbvterm{s}}{\intertype{\functtype{\M}{\sigma}}{}}}$.
      Then, by \ih
      $\sequV{\Gamma'}{\assign{s}{\intertype{\functtype{\M}{\sigma}}{}}}$
      and $\sequV{\Delta}{\assign{u}{\M}}$. Finally, we conclude by rule
      $\ruleVArrowE$.
    \end{itemize}
    
    \item $t = \termabs{x}{s}$. Then, $\cbvterm{t} =
    \termbang{\termabs{x}{\cbvterm{s}}}$, $\sigma = \intertype{\sigma_i}{i \in I}$,
    $\Gamma = \ctxtsum{}{\Gamma_i}{i \in I}$ and
    $\many{\sequB{\Gamma_i}{\assign{\termabs{x}{\cbvterm{s}}}{\sigma_i}}}{i \in I}$.
    Moreover, by rule $\ruleBArrowI$, for every $i \in I$ we have $\sigma_i =
    \functtype{\Gamma'_i(x)}{\tau_i}$, $\Gamma_i = \ctxtres{\Gamma'_i}{x}{}$
    and $\sequB{\Gamma'_i}{\assign{\cbvterm{s}}{\tau_i}}$. By \ih
    $\many{\sequV{\Gamma'_i}{\assign{s}{\tau_i}}}{i \in I}$ and we conclude by
    rule $\ruleVArrowI$.
    
    \item $t = \termsubs{x}{u}{s}$. Then, $\cbvterm{t} =
    \termsubs{x}{\cbvterm{u}}{\cbvterm{s}}$, $\Gamma =
    \ctxtsum{(\ctxtres{\Gamma'}{x}{})}{\Delta}{}$,
    $\sequB{\Gamma'}{\assign{\cbvterm{s}}{\sigma}}$ and
    $\sequB{\Delta}{\assign{\cbvterm{u}}{\Gamma'(x)}}$. The result follow
    immediately from the \ih using rule $\ruleVESubs$.
  \end{itemize}
\end{enumerate}
\end{proof}



==> proofs/cbn-cbv-substitution.tex <==
\begin{proof} \mbox{}
\begin{enumerate}
  \item By induction on $t$.
  \begin{itemize}
    \item $t = x$. Then, $\cbnterm{\substitute{x}{u}{x}} = \cbnterm{u} =
    \substitute{x}{\cbnterm{u}}{x} = \substitute{x}{\cbnterm{u}}{\cbnterm{x}}$.
    
    \item $t = y$. Then, $\cbnterm{\substitute{x}{u}{y}} = y =
    \substitute{x}{\cbnterm{u}}{y} = \substitute{x}{\cbnterm{u}}{\cbnterm{y}}$.
    
    \item $t = \termapp{t_0}{t_1}$. Then, \[
\begin{array}{rll}
\cbnterm{\substitute{x}{u}{(t_0 t_1)}}
 & =              & \cbnterm{(\termapp{\substitute{x}{u}{t_0}}{\substitute{x}{u}{t_1}})} \\
 & =              & \termapp{\cbnterm{\substitute{x}{u}{t_0}}}{\termbang{(\cbnterm{\substitute{x}{u}{t_1}})}} \\
 & =_{\text{\ih}} & \termapp{\substitute{x}{\cbnterm{u}}{\cbnterm{t_0}}}{\termbang{\substitute{x}{\cbnterm{u}}{\cbnterm{t_1}}}} \\
 & =              & \substitute{x}{\cbnterm{u}}{(\termapp{\cbnterm{t_0}}{\termbang{\cbnterm{t_1}}})} \\
 & =              & \substitute{x}{\cbnterm{u}}{\cbnterm{(\termapp{t_0}{t_1})}}
\end{array} \]
    
    \item $t = \termabs{y}{t_0}$. Straightforward by the \ih
    
    \item $t = \termsubs{y}{t_1}{t_0}$. Similar to the previous case. 
  \end{itemize}
  
  \item By induction on $t$.
  \begin{itemize}
    \item $t = x$. Then, $\cbvterm{\substitute{x}{v}{x}} = \cbvterm{v} = \termbang{u} =
    \substitute{x}{u}{(\termbang{x})} = \substitute{x}{u}{\cbvterm{x}}$.
    
    \item $t = y$. Then, $\cbvterm{\substitute{x}{v}{y}} = \cbvterm{y} =
    \substitute{x}{u}{\cbvterm{y}}$.
    
    \item $t = \termapp{t_0}{t_1}$. There are two cases:
    \begin{itemize}
      \item If $\cbvterm{t_0} = \ctxtapp{\ctxt{L}}{\termbang{s}}$,
      then the \ih gives $\cbvterm{\substitute{x}{v}{t_0}} =
      \substitute{x}{u}{\cbvterm{t_0}} =
      \substitute{x}{u}{\ctxtapp{\ctxt{L}}{\termbang{s}}} =
      \ctxtapp{\substitute{x}{u}{\ctxt{L}}}{\termbang{\substitute{x}{u}{s}}}$.
      Then, \[
\begin{array}{rll}
\cbvterm{\substitute{x}{v}{(\termapp{t_0}{t_1})}}
 & =              & \cbvterm{(\termapp{\substitute{x}{v}{t_0}}{\substitute{x}{v}{t_1}})} \\
 & =              & \termapp{\ctxtapp{\substitute{x}{u}{\ctxt{L}}}{\substitute{x}{u}{s}}}{\cbvterm{(\substitute{x}{v}{t_1})}} \\
 & =_{\text{\ih}} & \termapp{\ctxtapp{\substitute{x}{u}{\ctxt{L}}}{\substitute{x}{u}{s}}}{(\substitute{x}{u}{\cbvterm{t_1}})} \\
 & =              & \substitute{x}{u}{\termapp{\ctxtapp{\ctxt{L}}{s}}{\cbvterm{t_1}}} \\
 & =              & \substitute{x}{u}{\cbvterm{(\termapp{t_0}{t_1})}}
\end{array} \]
      
      \item Otherwise, $\cbvterm{\substitute{x}{v}{(\termapp{t_0}{t_1})}} =
      \cbvterm{(\termapp{\substitute{x}{v}{t_0}}{\substitute{x}{v}{t_1}})}$. The
      \ih gives $\cbvterm{\substitute{x}{v}{t_0}} = \substitute{x}{u}{\cbvterm{t_0}}$
      and $\cbvterm{\substitute{x}{v}{t_1}} = \substitute{x}{u}{\cbvterm{t_1}}$.
      Moreover, $\cbvterm{t_0} \neq \ctxtapp{\ctxt{L}}{\termbang{s}}$ implies the
      same for $\substitute{x}{u}{\cbvterm{t_0}}$, simply because $u$ is a variable
      or an abstraction. Then, \[
\begin{array}{rll}
\cbvterm{(\termapp{\substitute{x}{v}{t_0}}{\substitute{x}{v}{t_1}})}
 & = & \termapp{\termder{(\substitute{x}{u}{\cbvterm{t_0}})}}{\substitute{x}{u}{\cbvterm{t_1}}} \\
 & = & \substitute{x}{u}{(\termapp{\termder{(\cbvterm{t_0})}}{\cbvterm{t_1}})} \\
 & = & \substitute{x}{u}{\cbvterm{(\termapp{t_0}{t_1})}}
\end{array} \]
    \end{itemize}
    
    \item $t = \termabs{y}{t_0}$. Then,\[
\begin{array}{rll}
\cbvterm{\substitute{x}{v}{(\termabs{y}{t_0})}}
 & =              & \cbvterm{(\termabs{y}{\substitute{x}{v}{t_0}})} \\
 & =              & \termbang{\termabs{y}{\cbvterm{(\substitute{x}{v}{t_0})}}} \\
 & =_{\text{\ih}} & \termbang{\termabs{y}{(\substitute{x}{u}{\cbvterm{t_0}})}} \\
 & =              & \substitute{x}{u}{\termbang{(\termabs{y}{\cbvterm{t_0}})}} \\
 & =              & \substitute{x}{u}{\cbvterm{(\termabs{y}{t_0})}}
\end{array} \]
    
    \item $t = \termsubs{y}{t_1}{t_0}$. This case is straightforward by the \ih
  \end{itemize}
\end{enumerate}
\end{proof}


==> proofs/cbvalue/cexp-variable.tex <==
\begin{proof}
$\Rightarrow$) By induction on $\Phi$ analysing the last rule applied.
\begin{itemize}
  \item $\ruleVTAxiom$, $\ruleVTArrowI$, $\ruleVTArrowN$, $\ruleVTArrowE$. Then
  $\Phi$ concludes with a non-multiset type. Hence these cases do not apply.

  \item $\ruleVTESubs$. Then $t = \termsubs{x}{u}{r}$, $\Gamma =
  \ctxtsum{\ctxtres{\Gamma'}{x}{}}{\Delta}{}$, $\cmult = \cmult_1 +
  \cmult_2$, $\cexp = \cexp_1 + \cexp_2$ and $\csize = \csize_1 + \csize_2$,
  and we have the type derivations
  $\derivable{\Phi_{r}}{\sequT{\Gamma'}{\assign{r}{\multiset{\typetight}}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTightCBV}$
  and
  $\derivable{\Phi_{u}}{\sequT{\Delta}{\assign{u}{\typeneutral}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTightCBV}$
  with $\ptight{\Gamma'(x)}$. Note that $\Gamma$ tight implies $\Gamma'$
  tight as well. Moreover, $\cexp = 1$ and Lem.~\ref{l:value:cexp-positive}
  imply $\cexp_1 = 1$. Hence, $\cmult_2 = \cexp_2 = 0$ and, by
  Lem.~\ref{l:value:tight-spreading} (\ref{l:value:tight-spreading:tight}), we
  have $u \in \HCBVNF$. By \ih with $\Phi_{r}$ we also get $r \in \VarHCBVNF$,
  thus it is safe to conclude $t \in \VarHCBVNF$.
  
  \item $\ruleVDAxiom$. Then $t = x \in \VarHCBVNF$ and the result is
  immediate.
  
  \item $\ruleVDArrowE$. \andres{TODO}
  
  \item $\ruleVDApp$. \andres{TODO}
  
  \item $\ruleVDArrowI$. This case does not apply since it concludes with a
  type of the form $\multiset{\functtype{\M}{\sigma}}$.
  
  \item $\ruleVDESubs$. \andres{TODO}
\end{itemize}

$\Leftarrow$) \andres{TODO}
\end{proof}



==> proofs/cbvalue/equivalence.tex <==
\begin{proof}
The fact that (\ref{l:value:equivalence:cbv}) implies
(\ref{l:value:equivalence:dv}) is straightforward since $\loredv$ is a
deterministic strategy for the calculus $\rewrite{\callbyvalue}$. Moreover,
(\ref{l:value:equivalence:cbv}) iff (\ref{l:value:equivalence:nf}) holds by
Lem.~\ref{l:value:normal-forms}. We show that (\ref{l:value:equivalence:dv})
implies (\ref{l:value:equivalence:nf}). For that, we prove simultaneously the
following statements:
\begin{enumerate}
  \item\label{l:value:equivalence:vr} If $t \not\loredv$ and $\neg\pabs{t}$ and
  $\neg\papp{t}$, then $t \in \VarHCBVNF$.
  
  \item\label{l:value:equivalence:ne} If $t \not\loredv$ and $\neg\pabs{t}$ and
  $\neg\pvar{t}$, then $t \in \HCBVNF$.
  
  \item\label{l:value:equivalence:no} If $t \not\loredv$, then $t \in \CBVNF$.
\end{enumerate}
\begin{enumerate}
  \item First of all notice that $\neg\pabs{t}$ and $\neg\papp{t}$ implies
  $\pvar{t}$. We have two cases to consider. 
  \begin{itemize}
    \item $t = x$. Then $t \in \VarHCBVNF$ is obvious. 
    
    \item $t = \termsubs{x}{u'}{u}$. Then $\neg\pval{u'}$, otherwise $t$ would
    be $\valuestg$-reducible, and also $u' \not\loredv$, otherwise $t$ would be
    $\valuestg$-reducible as well. Moreover, $\neg\pval{u'}$ implies
    $\neg\pabs{u'}$ and $\neg\pvar{u'}$. Then, the \ih
    (\ref{l:value:equivalence:ne}) gives $u' \in \HCBVNF$. Therefore, $u
    \not\loredv$, otherwise $t$ would be $\valuestg$-reducible. Also,
    $\pvar{t}$ implies $\pvar{u}$, which in turn implies $\neg\pabs{u}$ and
    $\neg\papp{u}$. Then, the \ih (\ref{l:value:equivalence:vr}) gives $u \in
    \VarHCBVNF$. This together with $u' \in \HCBVNF$ implies $t \in
    \VarHCBVNF$.
    
  \end{itemize}
  
  \item First of all notice that $\neg\pabs{t}$ and $\neg\pvar{t}$
  implies $\papp{t}$. We have two cases to consider.
  \begin{itemize}
    \item $t = \termapp{u}{u'}$. Then $\neg\pabs{u}$, otherwise $t$ would be
    $\valuestg$-reducible, and thus $u \not\loredv$, otherwise $t$ would be
    $\valuestg$-reducible. Thus in particular $\neg\pvar{u}$ or $\neg\papp{u}$.
    By the \ih (\ref{l:value:equivalence:vr}) or (\ref{l:value:equivalence:ne})
    we get $u \in  \VarHCBVNF \cup \HCBVNF$, so that $u' \not\loredv$,
    otherwise $t$ would be $\valuestg$-reducible. Then the \ih
    (\ref{l:value:equivalence:no}) gives $u' \in  \CBVNF$. This together with
    $u \in  \VarHCBVNF \cup \HCBVNF$ gives $t \in \HCBVNF$ as required.
     
    \item $t = \termsubs{x}{u'}{u}$. Then $\neg\pval{u'}$, otherwise $t$ would
    be $\valuestg$-reducible, and also $u' \not\loredv$, otherwise $t$ would be
    $\valuestg$-reducible as well. Moreover, $\neg\pval{u'}$ implies
    $\neg\pabs{u'}$ and $\neg\pvar{u'}$. Then, the \ih
    (\ref{l:value:equivalence:ne}) gives $u' \in \HCBVNF$. Therefore, $u
    \not\loredv$, otherwise $t$ would be $\valuestg$-reducible. Also,
    $\papp{t}$ implies $\papp{u}$, which in turn implies $\neg\pabs{u}$ and
    $\neg\pvar{u}$. Then, the \ih (\ref{l:value:equivalence:ne}) gives $u \in
    \HCBVNF$. This together with $u' \in \HCBVNF$ implies $t \in \HCBVNF$.
    
  \end{itemize}
  
  \item Let $t \not\loredv$. If $t = x$ or $t = \termabs{x}{u}$ the property is
  straightforward. If $t = \termapp{u}{u'}$, then $\neg\pabs{u}$, otherwise $t$
  would be $\valuestg$-reducible, and then $u \not\loredv$, otherwise $t$ would
  be $\valuestg$-reducible. Moreover, $\neg\pvar{u}$ or $\neg\papp{u}$. Thus
  the \ih (\ref{l:value:equivalence:vr}) or (\ref{l:value:equivalence:ne})
  gives $u \in \VarHCBVNF$ or $u \in \HCBVNF$ respectively. Therefore $u'
  \not\loredv$, otherwise $t$ would be $\valuestg$-reducible. The \ih
  (\ref{l:value:equivalence:no}) gives $u' \in \CBVNF$. This together with $u
  \in \VarHCBVNF$ or $u \in \HCBVNF$ gives $t \in \CBVNF$. If $t =
  \termsubs{x}{u'}{u}$, then $\neg\pval{u'}$, otherwise $t$ would be
  $\valuestg$-reducible. Moreover, $u' \not\loredv$, otherwise $t$
  would be $\valuestg$-reducible as well. Since $\neg\pval{u'}$ implies
  $\neg\pabs{u'}$ and $\neg\pvar{u'}$, by \ih (\ref{l:value:equivalence:ne})
  we have $u' \in \HCBVNF$. Then $u \not\loredv$, otherwise $t$ would be
  $\valuestg$-reducible. Thus the \ih (\ref{l:value:equivalence:no}) gives $u
  \in \CBVNF$. From $u \in \CBVNF$ and $u' \in \HCBVNF$ we conclude $t \in
  \CBVNF$.
\end{enumerate}
\end{proof}



==> proofs/cbvalue/normal-typable.tex <==
\begin{proof}
By simultaneous induction on the following claims: \andres{TODO: adaptar!}
\begin{enumerate}
  \item\label{t:clashfree-bang:ne} $t \in \VarHCBVNF$ iff $\derivable{\Phi}{\sequB{\Gamma}{\assign{t}{??}}}{\SysTightCBV}$.
  \item\label{t:clashfree-bang:na} $t \in \HCBVNF$ iff there exists $\derivable{\Phi}{\sequB{\Gamma}{\assign{t}{\M}}}{\SysTightCBV}$.
  \item\label{t:clashfree-bang:nb} $t \in \CBVNF$ iff there exists $\derivable{\Phi}{\sequB{\Gamma}{\assign{t}{\tau}}}{\SysTightCBV}$.
 \end{enumerate}
We first show the left-to-right implications by only analysing the key cases.
If $t =
\cfntrl{x}$, then $\pntrl{t}$ and for every type $\tau$ we conclude by
$\ruleBAxiom$. If $t = \cfntrl{\termapp{s}{u}}$, by definition
$\cfntrl{s}$ and $\cfnabs{u}$. Let $\tau$ be any type. By \ih
(\ref{t:clashfree-bang:na}) $\pnabs{u}$ and
$\derivable{}{\sequB{\Delta}{\assign{u}{\M}}}{\SysBang}$. Then, by \ih
(\ref{t:clashfree-bang:ne}) we get $\pntrl{s}$ and
$\derivable{}{\sequB{\Gamma}{\assign{s}{\functtype{\M}{\tau}}}}{\SysBang}$.
Moreover, $\pntrl{s}$ and $\pnabs{u}$ imply $\pnabs{s}$ and
$\pnrml{u}$ resp., hence $\pntrl{t}$. Thus, we conclude by
$\ruleBArrowE$,
$\derivable{\Phi}{\sequB{\ctxtsum{\Gamma}{\Delta}{}}{\assign{\termapp{s}{u}}{\tau}}}{\SysBang}$.
If $t = \cfnbang{\termabs{x}{s}}$, then $\cfnrml{s}$ by definition. By
\ih (\ref{t:clashfree-bang:no}) $\pnrml{s}$ and
$\derivable{}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}$ for some
type $\tau$. Then, $\pnbang{t}$ and we conclude by $\ruleBArrowI$,
$\derivable{\Phi}{\sequB{\ctxtres{\Gamma}{x}{}}{\assign{\termabs{x}{s}}{\functtype{\Gamma(x)}{\tau}}}}{\SysBang}$.
If $t = \cfnabs{\termbang{s}}$, then $\pnabs{t}$ by definition and we
conclude by $\ruleBBang$,
$\derivable{\Phi}{\sequB{}{\assign{\termbang{s}}{\emul}}}{\SysBang}$. If
$t = \cfntrl{\termder{(s)}}$, then $\cfntrl{s}$ by definition. Let
$\tau$ be any type, by \ih (\ref{t:clashfree-bang:ne}) we get $\pntrl{s}$ and
$\derivable{}{\sequB{\Gamma}{\assign{s}{\multiset{\tau}}}}{\SysBang}$.
Moreover, $\pntrl{s}$ implies $\pnbang{s}$ and hence
$\pntrl{t}$. Thus, we conclude by $\ruleBDer$,
$\derivable{}{\sequB{\Gamma}{\assign{\termder{(s)}}{\tau}}}{\SysBang}$. If
$t = \termsubs{x}{u}{s}$, then $\cfntrl{u}$ and there are three
possible cases: $\cfntrl{s}$, $\cfnabs{s}$ or $\cfnbang{s}$. In either
case, by the proper \ih we get
$\derivable{}{\sequB{\Gamma}{\assign{s}{\tau}}}{\SysBang}$
(resp. $\M$) and conclude by $\ruleBESubs$, given that \ih (\ref{t:clashfree-bang:ne}) on $u$
implies $\pntrl{u}$ and
$\derivable{}{\sequB{\Delta}{\assign{u}{\Gamma(x)}}}{\SysBang}$. Note
that $\pntrl{u}$ in turn implies $\pnbang{u}$, thus $t$ remains
  in the same set as $s$ ($\ipntrl$, $\ipnabs$ or $\ipnbang$ resp.).

The right-to-left implications uses Lem.~\ref{l:clashfree-bang}.  
\end{proof}



==> proofs/cbvalue/split-value.tex <==
\begin{proof}
By case analysis on form of $v$.
\begin{itemize}
  \item $v = x$. By $\ruleDAxiom$, $\derivable{\Phi_v}{\sequTV{\assign{x}{\M}}{\assign{x}{\M}}{0}{1}{0}}{\SysCBV}$. From $\M =
  \ctxtsum{\!}{\M_i}{i \in I}$ we get
  $\many{\derivable{\Phi^i_{v}}{\sequTV{\assign{x}{\M_i}}{\assign{x}{\M_i}}{0}{1}{0}}{\SysCBV}}{i \in I}$ by
  $\ruleDAxiom$ several times, and conclude since $+_{i \in I} \cexp_i = |I|$.
  Note that the persistent rule $\ruleTAxiom$ does not apply since it does not
  conclude with a multiset type. 
  
  \item $v = \termabs{x}{s}$. By $\ruleDArrowI$, we have $\Gamma =
  \ctxtsum{\!}{\ctxtres{\Gamma_j}{x}{}}{j \in J}$, $\M =
  \intertype{\functtype{\Gamma_j(x)}{\tau_j}}{j \in J}$, $\cmult =
  +_{j \in J}{\cmult_j}$, $\cexp = 1 +_{j \in J}{\cexp_j}$, $\csize =
  +_{j \in J}{\csize_i}$ and
  $\many{\derivable{\Phi^j_{s}}{\sequTV{\Gamma_j}{\assign{s}{\tau_j}}{\cmult_j}{\cexp_j}{\csize_j}}{\SysCBV}}{j \in J}$
  for some $J$. Let $I = +_{i \in I}{J_i}$. Then, $\M_i =
  \intertype{\functtype{\Gamma_j(x)}{\tau_j}}{j \in J_i}$ for each $i \in I$,
  and
  $\many{\derivable{\Phi^i_v}{\sequTV{\ctxtsum{\!}{\ctxtres{\Gamma_j}{x}{}}{j \in J_i}}{\assign{\termabs{x}{s}}{\M_i}}{+_{j \in J_i}{\cmult_j}}{1+_{j \in J_i}{\cexp_j}}{+_{j \in J_i}{\csize_i}}}{\SysCBV}}{i \in I}$
  by $\ruleDArrowI$ with each $J_i$. Finally, we conclude since:
  \begin{itemize}
    \item $\Gamma = \ctxtsum{\!}{\ctxtres{\Gamma_j}{x}{}}{j \in J} = \ctxtsum{\!}{(\ctxtsum{\!}{\ctxtres{\Gamma_j}{x}{}}{j \in J_i})}{i \in I}$
    \item $\cmult = +_{j \in J}{\cmult_j} = +_{i \in I}{(+_{j \in J_i}{\cmult_j})}$
    \item $\cexp = 1 +_{j \in J}{\cexp_j} = 1 +_{i \in I}{(1 +_{j \in J_i}{\cexp_j})} - |I|$
    \item $\csize = +_{j \in J}{\csize_j} = +_{i \in I}{(+_{j \in J_i}{\csize_j})}$
  \end{itemize}
  As before, the persistent rule $\ruleTArrowI$ does not apply.
\end{itemize}
\end{proof}



==> proofs/diamond.tex <==
\begin{proof}
The proof is by induction on $t$. To make easier the notations, we write $u\sL$
instead of $\ctxtapp{\ctxt{L}}{u}$, where $\sL$ is the list of substitutions of
the context $\ctxt{L}$. 

We only show the two interesting cases (root reductions), all the other ones
being straightforward:
\begin{itemize}
  \item $t = ((\lambda x'. t)\sL_1 \exsubs{x}{(\termbang{u})\sL_2} \sL_3) u'
  \rewrite{\dBeta} \termsubs{x'}{u'}{t}\sL_1 \exsubs{x}{(\termbang{u})\sL_2} \sL_3
  = t _1$ and $t \rewrite{\sBang} (((\lambda x'. t)\sL_1)\bsubstitute{x}{u} \sL_2 \sL_3) u'
  = ((\lambda x'. t\bsubstitute{x}{u}) (\sL_1 \bsubstitute{x}{u}) \sL_2 \sL_3) u' = t_2$.
  By $\alpha$-conversion we can assume $x \notin \fv{u'}$ so that
  by defining \[
  t_3 = \termsubs{x'}{u'}{t\bsubstitute{x}{u}} (\sL_1 \bsubstitute{x}{u})\sL_2 \sL_3 = \termsubs{x'}{u'}{t}\bsubstitute{x}{u} (\sL_1 \bsubstitute{x}{u})\sL_2 \sL_3
  \] we can close the diagram as follows: $t_1
  \rewrite{\sBang} t_3$ and $t_2 \rewrite{\dBeta} t_3$.
  
  \item $t = \termder{((\termbang{u'})\sL_1\exsubs{x}{(\termbang{u})\sL_2} \sL_3)}
  \rewrite{\dBang} u' \sL_1\exsubs{x}{(\termbang{u})\sL_2} \sL_3 = t_1$ and
  also $t \rewrite{\sBang} \termder{((\termbang{u'})\sL_1\bsubstitute{x}{u}\sL_2 \sL_3)}
  = t_2$. We close the diagram with $t_1 \rewrite{\sBang} t_3$ and $t_2
  \rewrite{\dBang} t_3$, where $t_3 = (u' \sL_1)\bsubstitute{x}{u} \sL_2 \sL_3 =
  u' \bsubstitute{x}{u} \sL_1 \bsubstitute{x}{u} \sL_2 \sL_3$. 
\end{itemize}
\end{proof}


==> proofs/tight-translations/gcbv-preservation.tex <==
\begin{proof}
By induction on $\Phi$ analysing the last rule applied.
\begin{itemize}
 \item $\ruleVTAxiomVar$. Then $\derivable{\Phi}{\sequT{\assign{x}{\multiset{\typevar}}}{\assign{x}{\typevar}}{0}{0}{0}}{\SysTightCBV}$. 
   and $\gcbvterm{t} = \termbang{x}$.  We conclude
   $\derivable{\Phi'}{\sequT{\assign{x}{\multiset{\typeneutral}}}{\assign{\termbang{x}}{\multiset{\typeneutral}}}{0}{1}{0}}{\SysTight}$ by
   using $\ruleBDAxiom$, then  $\ruleBDBang$. The counters are as expected
   since $\countgvr{\Phi} = 1$.
   
  \item $\ruleVTAxiom$. Then,
  $\derivable{\Phi}{\sequT{}{\assign{x}{\typevalue}}{0}{0}{0}}{\SysTightCBV}$
  and $\gcbvterm{t} = \termbang{x}$. We conclude  by
  $\ruleBTBang$ with
  $\derivable{\Phi'}{\sequT{}{\assign{\termbang{x}}{\typevalue}}{0}{0}{0}}{\SysTightCBV}$.
  Note that the counters are as expected since $\countgvr{\Phi} = 0$.
  
  \item $\ruleVTArrowI$. Then,
  $\derivable{\Phi}{\sequT{}{\assign{\termabs{x}{r}}{\typevalue}}{0}{0}{0}}{\SysTightCBV}$
  and $\gcbvterm{t} = \termbang{\termabs{x}{\gcbvterm{r}}}$. We conclude
  by $\ruleBTBang$ with
  $\derivable{\Phi'}{\sequT{}{\assign{\termbang{\termabs{x}{\gcbvterm{r}}}}{\typevalue}}{0}{0}{0}}{\SysTight}$.
  Note that the counters are as expected since $\countgvr{\Phi} = 0$.
  
  \item $\ruleVTArrowE$. Then, $t = \termapp{r}{u}$, $\sigma = \typeneutral$
  and $\Phi$ is of the form \[
\Rule{
  \derivable{\Phi_{r}}{\sequT{\Gamma_1}{\assign{r}{\overline{\typevalue}}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTightCBV}
  \quad
  \derivable{\Phi_{u}}{\sequT{\Gamma_2}{\assign{u}{\overline{\typevar}}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTightCBV}
}{
  \sequT{\ctxtsum{\Gamma_1}{\Gamma_2}{}}{\assign{\termapp{r}{u}}{\typeneutral}}{\cmult_1+\cmult_2}{\cexp_1+\cexp_2}{\csize_1+\csize_2+1}
}{\ruleVTArrowE}
  \] where $\cexp= \cexp_1+\cexp_2$. By the \ih we have
  $\derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\cbvtypepos{\overline{\typevalue}}}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}$
  and
  $\derivable{\Phi'_{u}}{\sequT{\cbvtypeneg{\Gamma_2}}{\assign{\gcbvterm{u}}{\cbvtypepos{\overline{\typevar}}}}{\cmult_2}{\cexp'_2}{\csize_2}}{\SysTight}$
  with $\cexp'_1 = \cexp_1 + \countgvr{\Phi_{r}}$ and $\cexp'_2 = \cexp_2 +
  \countgvr{\Phi_{u}}$. Moreover, since $u$ is typed with $\overline{\typevar}$,
  then it is typed with $\typeneutral$ or $\typevalue$, and thus
  $\cbvtypepos{\overline{\typevar}} = \overline{\typeabs}$. There are two
  possible cases for $\overline{\typevalue}$:
  \begin{enumerate}
    \item $\overline{\typevalue} = \typevar$. Then, with
    $\cbvtypepos{\overline{\typevalue}} = \multiset{\typeneutral}$. We conclude by
    applying $\ruleBDDer$ and $\ruleBTArrowE$ to derive $\Phi'$ as follows \[
\Rule{
  \Rule{
    \derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\multiset{\typeneutral}}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}
  }{
    \sequT{\cbvtypeneg{\Gamma_1}}{\assign{\termder{(\gcbvterm{r})}}{\typeneutral}}{\cmult_1}{\cexp'_1}{\csize_1}
  }{\ruleBDDer}
  \derivable{\Phi'_{u}}{\sequT{\cbvtypeneg{\Gamma_2}}{\assign{\gcbvterm{u}}{\overline{\typeabs}}}{\cmult_2}{\cexp'_2}{\csize_2}}{\SysTight}
}{
  \sequT{\cbvtypeneg{\Gamma}}{\assign{\gcbvterm{t}}{\typeneutral}}{\cmult}{\cexp'}{\csize}
}{\ruleBTArrowE}
    \] where $\cexp' = \cexp'_1 + \cexp'_2$. Hence, $\cexp' = \cexp'_1 +
    \cexp'_2 = \cexp_1 + \countgvr{\Phi_{r}} + \cexp_2 + \countgvr{\Phi_{u}} =
    \cexp + \countgvr{\Phi}$ as expected.
    
    \item $\overline{\typevalue} = \typeneutral$. Then, we have
    $\derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\typeneutral}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}$.
    We conclude by applying $\ruleBTDer$ and $\ruleBTArrowE$ to derive $\Phi'$
    as follows \[
\Rule{
  \Rule{
    \derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\typeneutral}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}
  }{
    \sequT{\cbvtypeneg{\Gamma_1}}{\assign{\termder{(\gcbvterm{r})}}{\typeneutral}}{\cmult_1}{\cexp'_1}{\csize_1}
  }{\ruleBTDer}
  \derivable{\Phi'_{u}}{\sequT{\cbvtypeneg{\Gamma_2}}{\assign{\gcbvterm{u}}{\overline{\typeabs}}}{\cmult_2}{\cexp'_2}{\csize_2}}{\SysTight}
}{
  \sequT{\cbvtypeneg{\Gamma}}{\assign{\gcbvterm{t}}{\typeneutral}}{\cmult}{\cexp'}{\csize}
}{\ruleBTArrowE}
    \] where $\cexp' = \cexp'_1 + \cexp'_2$. Hence, $\cexp' = \cexp'_1 +
    \cexp'_2 = \cexp_1 + \countgvr{\Phi_{r}} + \cexp_2 + \countgvr{\Phi_{u}} =
    \cexp + \countgvr{\Phi}$ as expected.
  \end{enumerate}
  
  \item $\ruleVTESubs$. Then, $t = \termsubs{x}{u}{r}$, $\sigma = \typetight$
  and $\Phi$ is of the form \[
\Rule{
  \derivable{\Phi_{r}}{\sequT{\Gamma_1}{\assign{r}{\typetight}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTightCBV}
  \quad
  \derivable{\Phi_{u}}{\sequT{\Gamma_2}{\assign{u}{\typeneutral}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTightCBV}
}{
  \sequT{\ctxtsum{\Gamma_1}{\Gamma_2}{}}{\assign{\termsubs{x}{u}{r}}{\typetight}}{\cmult_1+\cmult_2}{\cexp_1+\cexp_2}{\csize_1+\csize_2}
}{\ruleVTESubs}
  \] with $\ptight{\Gamma_1(x)}$ and $\cexp= \cexp_1+\cexp_2$. By the \ih on
  $\Phi_{u}$ there exists
  $\derivable{\Phi'_{u}}{\sequT{\cbvtypeneg{\Gamma_2}}{\assign{\gcbvterm{u}}{\typeneutral}}{\cmult_2}{\cexp'_2}{\csize_2}}{\SysTight}$
  with $\cexp'_2 = \cexp_2 + \countgvr{\Phi_{u}}$. By the \ih again there
  exists a derivation
  $\derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\cbvtypepos{\typetight}}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}$
  with $\cexp'_1 = \cexp_1 + \countgvr{\Phi_{r}}$. Thus, we conclude by applying
  $\ruleBTESubs$ with $\Phi'_{r}$, $\Phi'_{u}$ and $\ptight{\cbvtypeneg{\Gamma_1}(x)}$,
  hence obtaining the derivation
  $\derivable{\Phi'}{\sequT{\cbvtypeneg{\Gamma}}{\assign{\gcbvterm{t}}{\cbvtypepos{\typetight}}}{\cmult}{\cexp'}{\csize}}{\SysTight}$
  where $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1 + \countgvr{\Phi_{r}} + \cexp_2
  + \countgvr{\Phi_{u}} = \cexp + \countgvr{\Phi}$ as expected.
  
  \item $\ruleVDAxiom$. Then,
  $\derivable{\Phi}{\sequT{\assign{x}{\M}}{\assign{x}{\M}}{0}{1}{0}}{\SysTightCBV}$
  with $\M = \intertype{\sigma_i}{i \in I}$. We conclude
  by $\ruleBDAxiom$ and $\ruleBDBang$, deriving
  $\Phi'$ as follows \[
\Rule{
  \left(\hspace{-1em}\raisebox{-1em}{
    \Rule{}{
      \sequT{\assign{x}{\multiset{\cbvtypeneg{\sigma_i}}}}{\assign{x}{\cbvtypeneg{\sigma_i}}}{0}{0}{0}
    }{\ruleBDAxiom}
  }\hspace{-0.5em}\right)_{i \in I}
}{
  \sequT{\assign{x}{\cbvtypeneg{\M}}}{\assign{\termbang{x}}{\cbvtypeneg{\M}}}{0}{1}{0}
}{\ruleBDBang}
  \] Note that the counters are as expected since $\countgvr{\Phi} = 0$. We
  conclude since $\cbvtypeneg{\M}= \cbvtypepos{\M}$. 
  
  \item $\ruleVDArrowE$. Then $t = \termapp{r}{u}$, $\gcbvterm{t} =
  \termapp{\termder{(\gcbvterm{r})}}{\gcbvterm{u}}$, and $\Phi$ is of the form \[
\Rule{
  \derivable{\Phi_{r}}{\sequT{\Gamma_1}{\assign{r}{\multiset{\functtype{\M}{\sigma}}}}{\cmult_1}{\cexp_1}{\csize_1}}{\SysTightCBV}
  \quad
  \derivable{\Phi_{u}}{\sequT{\Gamma_2}{\assign{u}{\M}}{\cmult_2}{\cexp_2}{\csize_2}}{\SysTightCBV}
}{
  \sequT{\ctxtsum{\Gamma_1}{\Gamma_2}{}}{\assign{\termapp{r}{u}}{\sigma}}{\cmult_1+\cmult_2+1}{\cexp_1+\cexp_2-1}{\csize_1+\csize_2}
}{\ruleVDArrowE}
  \] where $\cmult = \cmult_1 + \cmult_2 + 1$, $\cexp = \cexp_1 + \cexp_2 - 1$,
  and $\csize = \csize_1 + \csize_2$. By the \ih on $\Phi_{u}$ there exists a
  derivation
  $\derivable{\Phi'_{u}}{\sequT{\cbvtypeneg{\Gamma_2}}{\assign{\gcbvterm{u}}{\cbvtypepos{\M}}}{\cmult_2}{\cexp'_2}{\csize_2}}{\SysTight}$
  with $\cexp'_2 = \cexp_2 + \countgvr{\Phi_{u}}$. And by the \ih on $\Phi_{r}$
  there exists
  $\derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\multiset{\functtype{\cbvtypeneg{\M}}{\cbvtypepos{\sigma}}}}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}$
  with $\cexp'_1 = \cexp_1 + \countgvr{\Phi_{r}}$. We conclude by deriving
  $\Phi'$ as follows \[
\Rule{
  \Rule{
    \derivable{\Phi'_{r}}{\sequT{\cbvtypeneg{\Gamma_1}}{\assign{\gcbvterm{r}}{\multiset{\functtype{\cbvtypeneg{\M}}{\cbvtypepos{\sigma}}}}}{\cmult_1}{\cexp'_1}{\csize_1}}{\SysTight}
  }{
    \sequT{\cbvtypeneg{\Gamma_1}}{\assign{\termder{(\gcbvterm{r})}}{\functtype{\cbvtypeneg{\M}}{\cbvtypepos{\sigma}}}}{\cmult_1}{\cexp'_1}{\csize_1}
  }{\ruleBDDer}
  \derivable{\Phi'_{u}}{\sequT{\cbvtypeneg{\Gamma_2}}{\assign{\gcbvterm{u}}{\cbvtypepos{\M}}}{\cmult_2}{\cexp'_2}{\csize_2}}{\SysTight}
}{
  \sequT{\cbvtypeneg{\Gamma}}{\assign{\gcbvterm{t}}{\cbvtypepos{\sigma}}}{\cmult}{\cexp'}{\csize}
}{\ruleBDArrowE}
  \] where $\cexp' = \cexp'_1 + \cexp'_2 = \cexp_1 + \countgvr{\Phi_{r}} +
  \cexp_2 + \countgvr{\Phi_{u}} = \cexp + 1 + \countgvr{\Phi_{r}} +
  \countgvr{\Phi_{u}} = \cexp + \countgvr{\Phi}$ as expected.
  
  \item $\ruleVDApp$. This case is similar to the previous one.
  
  \item $\ruleVDArrowI$. Then, $t = \termabs{x}{r}$ and $\Phi$ is of the form \[
\Rule{
  \many{
    \derivable{\Phi_i}{\sequT{\Gamma_i}{\assign{r}{\tau_i}}{\cmult_i}{\cexp_i}{\csize_i}}{\SysTightCBV}
  }{i \in I}
}{
  \sequT{\ctxtsum{}{\ctxtres{\Gamma_i}{x}{}}{i \in I}}{\assign{\termabs{x}{r}}{\intertype{\functtype{\Gamma_i(x)}{\tau_i}}{i \in I}}}{+_{i \in I}{\cmult_i}}{1+_{i \in I}{\cexp_i}}{+_{i \in I}{\csize_i}}
}{\ruleVDArrowI}
  \] where $\cexp = 1 +_{i \in I}{\cexp_i}$. By the \ih there exists
  $\derivable{\Phi'_i}{\sequT{\cbvtypeneg{\Gamma_i}}{\assign{\gcbvterm{r}}{\cbvtypepos{\tau_i}}}{\cmult_i}{\cexp'_i}{\csize_i}}{\SysTight}$,
  where $\cexp'_i = \cexp_i + \countgvr{\Phi_{i}}$ for each $i \in I$. We then
  conclude by applying $\ruleBDArrowI$ and $\ruleBDBang$, hence deriving
  $\Phi'$ as follows \[
\Rule{
  \left(\hspace{-1em}\raisebox{-1em}{
    \Rule{
      \derivable{\Phi'_i}{\sequT{\cbvtypeneg{\Gamma_i}}{\assign{\gcbvterm{r}}{\cbvtypepos{\tau_i}}}{\cmult_i}{\cexp'_i}{\csize_i}}{\SysTight}
    }{
      \sequT{\ctxtres{\cbvtypeneg{\Gamma_i}}{x}{}}{\assign{\termabs{x}{\gcbvterm{r}}}{\functtype{\cbvtypeneg{\Gamma_i(x)}}{\cbvtypepos{\tau_i}}}}{\cmult_i}{\cexp'_i}{\csize_i}
    }{\ruleBDArrowI}
  }\hspace{-0.5em}\right)_{i \in I}
    }{
  \sequT{\ctxtsum{}{\ctxtres{\cbvtypeneg{\Gamma_i}}{x}{}}{i \in I}}{\assign{\gcbvterm{t}}{\cbvtypepos{\intertype{\functtype{\Gamma_i(x)}{\tau_i}}{i \in I}}}}{+_{i \in I}{\cmult_i}}{1+_{i \in I}{\cexp'_i}}{+_{i \in I}{\csize_i}}
}{\ruleBDBang}
  \] taking $\cexp' = 1 +_{i \in I}{\cexp'_i} = 1
  +_{i \in I}{(\cexp_i + \countgvr{\Phi_{i}})} = \cexp + \countgvr{\Phi}$ as
  expected.
  
  \item $\ruleVDESubs$. This case is similar to $\ruleVTESubs$.
\end{itemize}
\end{proof}


